Communication Lower Bounds of Bilinear Algorithms for Symmetric Tensor Contractions

We introduce a new theoretical framework for deriving lower bounds on data movement in bilinear algorithms. Bilinear algorithms are a general representation of fast algorithms for bilinear functions, which include computation of matrix multiplication, convolution, and symmetric tensor contractions. A bilinear algorithm is described by three matrices. Our communication lower bounds are based on quantifying the minimal matrix ranks of matching subsets of columns of these matrices. This infrastructure yields new communication lower bounds for symmetric tensor contraction algorithms, which provide qualitative new insights. Tensor symmetry (invariance under permutation of modes) is common to many applications of tensor computations (e.g., tensor representation of hypergraphs, analysis of high order moments in data, as well as tensors modelling interactions of electrons in computational chemistry). Tensor symmetry enables reduction in representation size as well as arithmetic cost of contractions by factors that scale with the number of equivalent permutations. However, we derive lower bounds showing that these arithmetic cost and memory reductions can necessitate increases in data movement by factors that scale with the size of the tensors.

==> ack.tex <==
Solomonik was supported by a U.S. Department of Energy
Computational Science Graduate Fellowship
(DE-FG02-97ER25308) and an ETH Z\"urich Postdoctoral Fellowship.
%
Demmel was supported by the U.S. Department of Energy Office of Science, Office of Advanced Scientific Computing Research, Applied Mathematics program under awards: DE-SC0004938, DE-SC0003959, and DE-SC0010200 and 
%
by the U.S. Department of Energy Office of Science, Office of Advanced Scientific Computing Research, X-Stack program under awards: DE-SC0005136, DE-SC0008700, and AC02-05CH11231, 
%
and by DARPA award HR0011-12-2-0016.




==> apx.tex <==

\subsection{Proof of matrix multiplication communication lower bound}
\label{apx:seq_comm_lwb_mm}

We now give the proof for Theorem~\ref{thm:seq_comm_lwb_mm}.
\begin{proof}
The term $mk+kn+mn$ arises from the need to read the inputs into cache and write the output from
cache to main memory.

Consider the $mnk$ scalar multiplications done by any schedule which 
executes the matrix multiplication algorithm. If the schedule computes a contribution to $\C C$ more than
once, we only count  the contribution which gets written to the output in memory, and ignore any other
redundantly computed and discarded computation.
We subdivide the multiplications into $f$ chunks of size $\cachesize^{3/2}$ for 
$f= \lceil mnk/\cachesize^{3/2}\rceil$, with the last 'remainder' chunk being of size less than $\cachesize^{3/2}$ 
(we assume that $\cachesize^{3/2}$ does not divide evenly into $mnk$, so $mnk/\cachesize^{3/2} - \lfloor mnk/\cachesize^{3/2}\rfloor > 0$, the other case is strictly simpler). 
We can label each scalar multiplication $A_{il}\cdot B_{lj}$ 
with a tuple $(i,j,l)$. We then define three projections $\pi_1(i,j,l)=(j,l)$, $\pi_2(i,j,l)=(i,l)$,
and $\pi_3(i,j,l)=(i,j)$, which define the two operands needed by the $(i,j,l)$ multiplication and the entry
of the output $\C C$ to which the multiplication contributes. %\fixme{Edgar}{Need assumption that the contributions to $\C C$ are irreducible.} 
Given any set $S$ of tuples of size three, and projecting them onto a set of tuples of size two using
the three projections $\pi_m$, gives us sets 
$P_m=\{p : \exists s\in S,p\in \pi_m(s)\},\forall m\in\inti{1}{3}$.
By the regular Loomis-Whitney inequality~\cite{loomis1949n} inequality,
we obtain that $(|P_1| |P_2| |P_3|)^{1/2}\geq |S|$, from which it can be shown that $\sum_m |P_m|\geq 3|S|^{2/3}$. 
This inequality implies that for each chunk $i\in\inti{1}{f}$, which contains $t_i\leq \cachesize^{3/2}$ 
multiplications, at least $3t_i^{2/3}$  total operands of $\C A$ and $\B B$ plus contributions 
to $\C C$ are necessary (Lemma~\ref{thm:tlw} with $m=3$ and $r=2$ obtains a slightly smaller constant as it takes the union of the three projections).

Now, let $x_i$ be the number of operands present in cache prior to execution of chunk $i$
(by assumption $x_1=0$). The number of operands (elements of $\C A$ and $\C B$) 
present in cache at the end of execution of chunk $i$ should be equal to the number of 
operands available for chunk $i+1$, $x_{i+1}$. Let the number of contributions to $\C C$ (outputs),
which remain in cache (are not written to memory) at the end of chunk $i$, be $y_i$ 
(by assumption $y_f=0$), 
the rest of the outputs produced by chunk $i$ must be written to memory. In total, the amount
of reads from memory and writes to memory done during the execution of chunk $i$ with $t_i$ 
multiplications is then at least $w_i\geq 3t_i^{2/3}-x_i-y_i, \forall i\in \inti{1}{f}$. 
Now, since the operands and outputs 
which are kept in cache at the end of chunk $i$ must fit in cache, we know that for 
$i\in\inti{1}{f-1}, \ x_{i+1}+y_i\leq \cachesize$.
Substituting this in, we obtain $w_i\geq 3t_i^{2/3}-\cachesize-x_i+x_{i+1}, \forall i\in \inti{1}{f-1}$. 
Summing over all chunks yields a lower bound on the total communication cost, $\bwcost_\mathrm{MM}(m,n,k,\cachesize)$
\begin{align*}
\geq& \sum_{i=1}^f w_i \geq 3t_f^{2/3} - x_f + \sum_{i=1}^{f-1}(3t_i^{2/3}-\cachesize-x_i+x_{i+1}) \\
        =& -(f-1)\cachesize + 3t_f^{2/3} + \sum_{i=1}^{f-1} 3t_i^{2/3}  \\
        =& -(f-1)\cachesize + 3(mnk-(f-1)\cachesize^{3/2})^{2/3} + \sum_{i=1}^{f-1} 3\cachesize \\
        =& 2(f-1)\cachesize + 3(mnk-(f-1)\cachesize^{3/2})^{2/3} \\
        =& 2\cachesize\cdot \lfloor mnk/\cachesize^{3/2}\rfloor + 3(mnk-\lfloor mnk/\cachesize^{3/2}\rfloor\cdot \cachesize^{3/2})^{2/3}  \\
        =& 2mnk/\cachesize^{1/2} - 2\cachesize\cdot(mnk/\cachesize^{3/2} -\lfloor mnk/\cachesize^{3/2}\rfloor)  \\
        &+ 3\cachesize\cdot (mnk/\cachesize^{3/2}-\lfloor mnk/\cachesize^{3/2}\rfloor)^{2/3} \\
        \geq& 2mnk/\cachesize^{1/2} + 2\cachesize\cdot\bigg[(mnk/\cachesize^{3/2} \\
        &-\lfloor mnk/\cachesize^{3/2}\rfloor)^{2/3} - (mnk/\cachesize^{3/2}-\lfloor mnk/\cachesize^{3/2}\rfloor)\bigg] \\
        \geq& 2mnk/\cachesize^{1/2} 
\end{align*}
Therefore, we have
$$\bwcost_\mathrm{MM}(m,n,k,\cachesize)\geq \max\lt[\frac{2mnk}{\sqrt{\cachesize}},mk+kn+mn\rt].$$
\end{proof}
We note that a similar reduction may be used to show that the multiplication of nonsymmetric
matrices whose entries may overlap (e.g. $\C{A} \C{A}$) has cost no less than $\frac{\sqrt{2}}{4}$
of $\bwcost_\mathrm{MM}(n,m,k,\cachesize)$ (where it is assumed the entries $\C{A}$ and $\C{B}$ are disjoint/independent).


\subsection{Communication lower bounds for the direct evaluation algorithm}
In this section of the Appendix we give the reductions from sequential and parallel schedules for the direct evaluation algorithm for symmetric contractions to respective schedules for matrix multiplication.

\subsubsection{Vertical communication lower bound}
\label{apx:seq_comm_drct}

Here we give the proof of Theorem~\ref{thm:comm_lowerb_strd}, restated below.
\begin{theorem}
Let $q\defeq \max\lt({s+v\choose s},{v+t\choose t},{s+t \choose s}\rt)$,
any schedule of $\systalg ABstv$ on $\Gamma(\cs)$ has vertical communication cost,
%a sequential machine 
%with a cache of size $\cachesize$,
%i.e. the number of words moved between cache and memory,
%under the assumption that no operands start in cache and all outputs are 
%written to memory and that all elements have unit element size
%has the following bounds,
%is
\[\bwcost_\Psi(n,s,t,v,\cachesize) \geq \frac{1}{q}\bwcost_\mathrm{MM}\lt(\chchoose ns,\chchoose nt,\chchoose nv,q \cachesize\rt), \]
or if we expand the above and tighten the input/output lower bound slightly, $\bwcost_\Psi(n,s,t,v,\cachesize)$
%            & \frac{2n^{\omega}}{s!t!v!\sqrt{\cachesize}}&&+\frac{n^{s+t}}{s!t!} + \frac{n^{s+v}}{s!v!} + \frac{n^{v+t}}{t!v!} \geq 
\[\geq \max\bigg[\frac{1}{q^{3/2}}\frac{2n^{\omega}}{s!t!v!\sqrt{\cachesize}}, 
               \frac{n^{s+t}}{(s+t)!}+ \frac{n^{s+v}}{(s+v)!}+ \frac{n^{v+t}}{(v+t)!}\bigg].\]
\end{theorem}
\begin{proof}
The lower bound for reading in the
inputs from memory to cache and writing the output from cache to memory is
$$\bwcost_\Psi(n,s,t,v,\cachesize)\geq \frac{n^{s+t}}{(s+t)!}+ \frac{n^{s+v}}{(s+v)!}+ \frac{n^{v+t}}{(v+t)!},$$
which is lower than the corresponding lower bound
for nonsymmetric matrix multiplication, because the tensors have less unique entries than the corresponding matrices (the largest tensor by a factor of $q$).

Consider any schedule $\mathcal{S}$ for the direct evaluation symmetric contraction algorithm. We ignore the scaling 
by $s!t!$ and by $\rho(\tpl{k}{v})$ done by the algorithm, and we also ignore the accumulation of equivalent terms into entries of $\B C$ with
equivalent indices, by replacing the collection $\prt st(\tpl{i}{s+t})$ with a set $\bprt st(\tpl{i}{s+t})$ defined the same way except now without repeated entries.
Ignoring part of the computation still allows us to obtain a communication lower bound based on the cost of performing the rest of the computation.
The leftover operations in $\mathcal{S}$ compute $\forall \tpl{i}{s+t}\in\enti{1}{n}{s+t}$,
\[C_{\tpl{i}{s+t}}=  \sum_{(\tpl js,\tpl lt)\in \bprt st(\tpl{i}{s+t})} \bigg(\sum_{\tpl kv\in\enti 1nv} A_{\tpl js\tpl kv}\cdot B_{\tpl kv\tpl lt}\bigg),\]
where $\B A$ and $\B B$ are symmetric. We now show that the existence of $\mathcal S$ implies the existence of a schedule $\hat{\mathcal{S}}$, 
which computes $\forall \tpl{j}{s}\in\enti{1}{n}{s}, \tpl lt \in \enti 1nt$,
\[\hat{C}_{\tpl js \tpl lt}=  \sum_{\tpl kv\in\enti 1nv} \hat{A}_{\tpl js\tpl kv}\cdot \hat{B}_{\tpl kv\tpl lt},\]
for any $\BH A$ and $\BH B$ that are partially symmetric ($\BH A$ in the first $s$ and the last $v$ indices and $\BH B$ in the first $v$ and last $t$ indices).
We will show that $\hat{\mathcal{S}}$ requires a factor of $q$
%\[r=\max\lt(\frac{(s+v)!}{s!v!},\frac{(v+t)!}{t!v!},\frac{(s+t)!}{s!t!}\rt)\]
%\[r=\max\lt({s+v\choose s},{v+t\choose t},{s+t \choose s}\rt)\]
larger cache size and communication cost than $\mathcal{S}$. Then due to the fact that a the partially symmetric contraction above can be used to compute a matrix multiplication,
we will obtain the communication lower bound stated in the theorem.

The construction of $\hat{\mathcal S}$ from $\mathcal S$ works by associating a set of up ${s+v\choose s}$ elements of $\BH A$ with each element of $\B A$, $\forall \tpl{i_1}{s+v}\in \enti 1n{s+v}$,  
\[\mathring{A}_{\tpl{i_1}{s+v}}= \{\hat{A}_{\tpl{j}{s}\tpl{k}{v}} : (\tpl{j}{s},\tpl{k}{v})\in \bprt sv(\tpl{i_1}{s+v})\},\]
and a set of up to ${v+t \choose v}$ elements of $\BH B$ with each element of $\B B$, $\forall \tpl{i_2}{v+t}\in \enti 1n{v+t}$, 
\[\mathring{B}_{\tpl{i_2}{v+t}}= \{\hat{B}_{\tpl{k}{v}\tpl{l}{t}} : (\tpl{k}{v},\tpl{l}{t})\in \bprt vt(\tpl{i_2}{v+t})\}.\]
%Every read of an element of $\C A$ or $\C B$ from memory to cache in $\mathcal S$ (or any overwrite/discard of the element while inside cache) is replaced by a corresponding operation of 
%the corresponding element $\B{\mathring A}$ and

Every result of scalar multiplication and every partial sum of these must contribute to a unique element of $\B C$, i.e. $C_\tpl{i}{s+t}$ for some $\tpl{i}{s+t}$. %\in \enti{1}{n}{s+t}$.
Now, in $\mathcal S$, %$\forall \tpl{i}{s+t}\in \enti 1n{s+t}, 
each $C_\tpl{i}{s+t}$ is computed as a summation of $\chchoose{n}{v}$ multiplications, via $\chchoose{n}{v}{-}1$ addition operations.
Thus including $C_\tpl{i}{s+t}$ there are a total of $2\chchoose nv$ partial sums in $\mathcal S$ associated with each $C_\tpl{i}{s+t}$. We enumerate these as $C^{(g)}_\tpl{i}{s+t}$ for 
$g\in\inti{1}{2\chchoose nv}$. 
%\fixed{Edgar}{How many are there for diagonal elements?}
Further, any addition operation in $\mathcal S$ can be written for some $g,f_1,f_2\in \inti{1}{2\chchoose nv}$ and some $\tpl{i}{s+t}\in \enti{1}n{s+t}$ as
\[C^{(g)}_\tpl{i}{s+t}=C^{(f_1)}_\tpl{i}{s+t}+C^{(f_2)}_\tpl{i}{s+t}.\]
%We now associate a set of up to ${s+t \choose s}$ elements with each of these partial summations $C^{(h)}$

Every multiplication in $\mathcal S$ may be represented as
\[C^{(g)}_\tpl{i}{s+t}=A_\tpl{i_1}{s+v}\cdot B_\tpl{i_2}{v+t},\]
for some $\tpl{i_1}{s+v}\in\enti 1n{s+v} , \tpl{i_2}{v+t}\in\enti 1n{v+t}, g\in \inti{1}{2\chchoose nv}$.
For each partial sum $C^{(g)}_\tpl{i}{s+t}$, we now define a set of ${s+t \choose s}$ partial sums in $\hat{\mathcal S}$, % by associating a set of up to ${s+t\choose s}$ partial sums 
\[\mathring{C}^{(g)}_\tpl{i}{s+t}=\{\hat{C}^{(g)}_{\tpl js\tpl lt} : (\tpl{j}{s},\tpl{l}{t})\in\bprt st(\tpl{i}{s+t})\}.\]
For every scalar multiplication in $\mathcal S$, $C^{(g)}_\tpl{i}{s+t} = A_\tpl{i_1}{s+v}\cdot B_\tpl{i_2}{v+t}$, 
%there exist unique $\tpl{j}{s}\in \enti 1ns,\tpl{k}{v}\in \enti 1nv,\tpl{l}{t}\in \enti 1nt$ such that $(\tpl js,\tpl kv)\in \chi(\tpl{i_1}{s+v})$ and $(\tpl kv, \tpl lt) \in \chi(\tpl{i_2}{v+t})$.
there exist unique $\tpl{j}{s}$, $\tpl{k}{v}$, and $\tpl{l}{t}$ such that $(\tpl js,\tpl kv)\in \bprt sv(\tpl{i_1}{s+v})$ and $(\tpl kv, \tpl lt) \in \bprt vt(\tpl{i_2}{v+t})$.
\fixed{Edgar}{What about diagonal elements?}
For each such multiplication, schedule $\mathcal{\hat S}$ computes $\hat{C}^{(g)}_{\tpl js\tpl lt}=\hat{A}_{\tpl js \tpl kv}\cdot \hat{B}_{\tpl kv \tpl lt}$ and sets all the other elements of the set to which the result belongs,
$\mathring{C}^{(g)}_\tpl{i}{s+t}$, to zero.
For every addition $C^{(g)}_\tpl{i}{s+t}=C^{(f_1)}_\tpl{i}{s+t}+C^{(f_2)}_\tpl{i}{s+t},$ schedule $\hat{S}$ computes $\mathring{C}^{(g)}_\tpl{i}{s+t}$ via the additions:
\[\hat{C}^{(g)}_{\tpl js\tpl lt}=\hat{C}^{(f_1)}_{\tpl js\tpl lt}+\hat{C}^{(f_2)}_{\tpl js \tpl lt}\] 
for all elements in $\mathring{C}^{(f_1)}_\tpl{i}{s+t}$ and $\mathring{C}^{(f_2)}_\tpl{i}{s+t}$, respectively.
Schedule $\mathcal{\hat S}$ manages memory to cache traffic by mimicking $\mathcal S$.
Whenever an element of the form $A_\tpl{i_1}{s+v}$ or $B_\tpl{i_2}{v+t}$ or $C^{(g)}_\tpl{i}{s+t}$ is read from memory
to cache, $\mathcal{\hat S}$ reads one of the sets  $\mathring{A}_\tpl{i_1}{s+v}$ or $\mathring{B}_\tpl{i_2}{v+t}$ or $\mathring{C}^{(g)}_\tpl{i}{s+t}$, respectively.
Writes from memory to cache of $C^{(g)}_\tpl{i}{s+t}$ are similarly mimicked by writes of the set $\mathring{C}^{(g)}_\tpl{i}{s+t}$.

We prove correctness of schedule $\mathcal{\hat{S}}$ by demonstrating that if an element $C^{(g)}_\tpl{i}{s+t}=C_\tpl{i}{s+t}$ then 
\[\mathring{C}^{(g)}_\tpl{i}{s+t}=\{\hat{C}_{\tpl{j}{s}\tpl{l}{t}} :(\tpl{j}{s},\tpl{l}{t})\in\bprt st(\tpl{i}{s+t}) \},\]
and by arguing that all operands necessary are always present. 
It is easy to see that any operands to a multiplication or addition will be present.
For each addition with an operand $C^{(g)}_\tpl{i}{s+t}$ in $\mathcal S$, an addition is done
with members of $\mathring{C}^{(g)}_\tpl{i}{s+t}$ in $\mathcal{\hat S}$ and the communication of this set mimics that of $C^{(g)}_\tpl{i}{s+t}$.
Each multiplication in $\mathcal S$ is also mimicked by a multiplications of $\mathcal{\hat S}$, as well as the communication of the operands.

We can represent each partial sum as
\[C^{(g)}_{\tpl{i}{s+t}} = \sum_{(\tpl{j}{s},\tpl{l}{t})\in P} \bigg(\sum_{\tpl{k}{v}\in N_{\tpl{j}{s}\tpl{l}{t}}} A_{\tpl js\tpl kv}\cdot B_{\tpl kv\tpl lt}\bigg),\]
where $P\subseteq\bprt st(\tpl{i}{s+t})$ and each $N_{\tpl{j}{s}\tpl{l}{t}}\subseteq \enti 1nv$.
For each such $C^{(g)}_{\tpl{i}{s+t}}$, we show by induction that $\forall (\tpl{j}{s},\tpl{l}{t})\in P$,
\[\hat{C}^{(g)}_{\tpl{j}{s}\tpl{l}{t}} = \sum_{\tpl{k}{v}\in N_{\tpl{j}{s}\tpl{l}{t}}} A_{\tpl js\tpl kv}\cdot B_{\tpl kv\tpl lt}.\]
Each $C^{(g)}_{\tpl{i}{s+t}}$ is either a result of a multiplication (a leaf node in the summation tree) or a summation of two other such partial sums (an internal node in the summation tree).
For leaf nodes that are a result of a multiplication, $P$ contains a single element $(\tpl{j}{s},\tpl{l}{t})$ for some $\tpl js\in \enti 1ns$ and $\tpl lt \in \enti 1nv$,
and there is a single $\tpl kv\in N_{\tpl js\tpl lt}$.
This exact multiplication is performed in $\mathcal{S}$ to form $\hat{C}^{(g)}_{\tpl{j}{s}\tpl{l}{t}}$.
For any internal node that is a result of a summation $C^{(g)}_{\tpl{i}{s+t}}=C^{(f_1)}_\tpl{i}{s+t}+C^{(f_2)}_\tpl{i}{s+t}$, we can assert by induction that the 
%We need to show that $\mathring C^{(g)}_\tpl{i}{s+t}$ corrects the properly partitioned set of $C^{(g)}_{\tpl{j}{s}\tpl lt}$ which correspond to element of $\B C$ summed in $C^{(g)}_{\tpl{i}{s+t}}$
desired property holds for $\mathring{C}^{(f_1)}_\tpl{i}{s+t}$ (with $P^{f_1}$ and $N^{f_1}$) %(\tpl{j}{s},\tpl{l}{t})$) 
as well as for $\mathring{C}^{(f_2)}_\tpl{i}{s+t}$ (with $P^{f_2}$ and $N^{f_2}$).  %(\tpl{j}{s},\tpl{l}{t})$).
%nd since the elements corresponding to the same $(\tpl{j}{s},\tpl{l}{t})\in\bprt(\tpl{i}{s+t})$,
%we obtain 
For each $(\tpl{j}{s},\tpl{l}{t})\in P^{f_1} \cap P^{f_2}$, the elements are summed by $\mathcal S$, so we obtain the appropriate union,
\begin{align*}
\hat{C}^{(g)}_{\tpl{j}{s}\tpl{l}{t}} &= \hat{C}^{(f_1)}_{\tpl{j}{s}\tpl{l}{t}} + \hat{C}^{(f_2)}_{\tpl{j}{s}\tpl{l}{t}} \\
&=\sum_{\tpl{k}{v}\in \lt(N^{f_1}_{\tpl{j}{s}\tpl{l}{t}}\cup N^{f_2}_{\tpl{j}{s}\tpl{l}{t}}\rt)} A_{\tpl js\tpl kv}\cdot B_{\tpl kv\tpl lt}.
\end{align*}
Thus for each $(\tpl{j}{s},\tpl{l}{t})\in P^{f_1} \cap P^{f_2}$, we have $N^g_{\tpl{j}{s}\tpl{l}{t}}=N^{f_1}_{\tpl{j}{s}\tpl{l}{t}}\cup N^{f_2}_{\tpl js \tpl lt}$.
It is also easy to see that the property is preserved for $(\tpl{j}{s},\tpl{l}{t})\in P^{f_1} \setminus P^{f_2}$, %\cup P^g)\setminus (P^f \cap P^g)$,
where each $N^g_{\tpl{j}{s}\tpl{l}{t}}$ is equal to $N^{f_1}_{\tpl{j}{s}\tpl{l}{t}}$, since the elements are added to zero and similarly for $P^{f_2}\setminus P^{f_2}$.
% or $N^f_{\tpl{j}{s}\tpl{l}{t}}$.
Thus, we have shown the property holds with the appropriate $P^{g}=P^{f_1}\cup P^{f_2}$ and with $N^g$ as defined above. 
Whenever $C^{(g)}_{\tpl i{s+t}}=C_\tpl{i}{s+t}$, this property implies that $P = \bprt st(\tpl{i}{s+t})$ and also that $\forall (\tpl js, \tpl lt)\in\bprt st(\tpl i{s+t})$, $N_{\tpl js\tpl lt}=\enti 1nv$,
\[\hat{C}^{(g)}_{\tpl{j}{s}\tpl{l}{t}} = \sum_{\tpl{k}{v}\in \enti 1nv} A_{\tpl js\tpl kv}\cdot B_{\tpl kv\tpl lt}.\]

\fixed{Edgar}{This is not quite complete, we constructed a $P^g$ and $N^g$, but why are they the right ones? Not sure if its worth being even more verbose here, correctness of the construction should be evident.}
%We know that $\forall \tpl{i}{s+t}\in\enti 1n{s+t}$, 
%\[C_\tpl{i}{s+t}=\sum_{(\tpl js,\tpl lt)\in \chi(\tpl{i}{s+t})} \lt(\sum_{\tpl kv\in\enti 1nv} A_{\tpl js\tpl kv}\cdot B_{\tpl kv\tpl lt}\rt),\]
%and that each multiplication $A_{\tpl js\tpl kv}\cdot B_{\tpl kv\tpl lt}$ defines an element indexed by $\tpl js\tpl lt$ in some $\mathring{C}^{(g)}_\tpl{i}{s+t}$.
%Now, each $\mathring{C}^{(g)}_\tpl{i}{s+t}$ is in a summation tree whose leaves include $\hat{A}_{\tpl js\tpl {k'}v}\cdot \hat{B}_{\tpl {k'}v\tpl lt}, \forall \tpl {k'}v\in \enti 1nv$, because
%$A_{\tpl js\tpl {k'}v}\cdot B_{\tpl {k'}v\tpl lt}, \forall \tpl {k'}v\in \enti 1nv$ contributes to $C_\tpl{i}{s+t}$ as does $C^{(g)}_\tpl{i}{s+t}$.
%Since each addition of a partial sum contributing




%
%
%, which computes
%$\C{\bar{C}}=\C{\bar{A}} \C{\bar{B}}$, where $\C{\bar{A}}$ and $\C{\bar{B}}$ are matrices corresponding to folded forms
%of $\C A$ and $\C B$ respectively, and $\C{\bar{C}}$ is subsequently accumulated (symmetrized) to form $\C C$.
%We now construct a schedule $\bar{\mathcal{S}}$ that
%
%
%
%
%When these tensors all fit into cache, the above lower bound is attainable
%since the unique entries of $\C A$, $\C B$ can all be read into cache
%then contracted and symmetrized into $\C C$ on the fly. This cost is a factor of
%$(s+t)!/(s!t!)$ smaller than the IO complexity of reading in a nonsymmetric (folded)
%$\C{\bar{A}}$ of dimensions $n^s/s!$ and $n^t/t!$, and similarly for the costs associated with
%$\C{\bar{B}}$ and $\C{\bar{C}}$. When the tensors do not fit in cache, the symmetry is more
%difficult to exploit in a general fashion so our algorithm (upper bound) does not attempt to.
%However, it is at least possible to lower the communication cost by exploiting 
%symmetry in one tensor if the other two tensors are vectors. 
%For instance in multiplying a 
%symmetric-matrix by a vector, we could pick out blocks from the lower triangle
%of the matrix, and multiply them by the two sets of vector entries, which the
%block and its symmetric reflection are multiplied by, contributing to two sets of 
%vector entries in the output. However, this does not generalize easily to the 
%$s,t,v\geq 1$ case, where reading in extra subsets of $\C B$ and $\C C$ counteracts
%with the cache reuse achieved by reading in a larger subset of $\C B$ and $\C C$.
%
%We do not attempt to prove that schedules cannot achieve extra reuse when 
%$s,t,v\geq 1$, and instead simply prove a looser lower
%bound that yields a similar fractional symmetric prefactor for any $s,t,v$,
%$\bwcost_\Psi(n,s,t,v,\cachesize)$
%\[ \geq \min\lt(\frac{s!v!}{(s+v)!},\frac{t!v!}{(v+t)!},\frac{s!t!}{(s+t)!}\rt)^{3/2}\frac{2n^{s+v+t}}{s!t!v!\sqrt{\cachesize}}.\]
%So, whether this lower bound is attainable for $s,t,v\geq 1$ or whether a tighter bound 
%may be proven remains an open question.
%
%We obtain this lower bound by reducing from schedules for the  
%direct evaluation symmetric tensor contraction algorithm to schedules for nonsymmetric matrix
%multiplication (with an appropriate prefactor). In particular, for
%$r=\max\lt(\frac{(s+v)!}{s!v!},\frac{(v+t)!}{t!v!},\frac{(s+t)!}{s!t!}\rt)$,
%we show that any schedule for the direct evaluation symmetric contraction algorithm
%with cost $\bwcost(n,s,t,v,\cachesize)$ yields a schedule for matrix multiplication of arbitrary
%nonsymmetric matrices $\C{\hat{A}}$ and $\C{\hat{B}}$ which uses $r\cachesize$ cache memory
%and attains the cost 
%\[\bwcost_\mathrm{MM}(n^s/s!,n^t/t!,n^v/v!,r \cachesize)\leq r \bwcost(n,s,t,v,\cachesize),\]
%where $\bwcost_\mathrm{MM}$ is the communication cost of nonsymmetric multiplication, for which
%we have a lower bound via Theorem~\ref{thm:seq_comm_lwb_mm}.
%
%Consider any schedule for the direct evaluation symmetric contraction algorithm, which computes
%$\C{\bar{C}}=\C{\bar{A}} \C{\bar{B}}$, where $\C{\bar{A}}$ and $\C{\bar{B}}$ are matrices corresponding to folded forms
%of $\C A$ and $\C B$ respectively, and $\C{\bar{C}}$ is subsequently accumulated (symmetrized) to form $\C C$.
%Such a schedule may employ multiplications of entries of the operands $A_{ij}\in \C{\bar{A}}$, which are equivalent to
%some other $A_{kl}\in \C{\bar{A}}$, $A_{ij}=A_{kl}$, due to being symmetric in $\C A$ (the folding ignores some symmetries),
%and the same for $\C B$.
%We represent the schedule as an interleaved sequence $S$ of `read', `write', `compute', `copy', and `discard' operations.
%We define cache storage set $M_l$ to be the elements stored in cache after the $i$th operation in the sequence $S$ and let $M_0=\emptyset$, since
%we assume the cache is empty at the start.
%The size of the cache storage set $\forall l\in\inti{1}{|S|}$, should not exceed the cache capacity $|M_l| \leq \cachesize$. 
%Any operations in sequence $s_l\in S$ must be one the following,
%\begin{itemize} 
%\item read of an element of $\C A$ from memory into cache, $s_l=(a,\mathrm{read})$, where $a\in \C A$ and $a \notin  M_{l-1}$, but subsequently $a\in M_l$,
%\item read of an element of $\C B$ from memory into cache, $s_l=(b,\mathrm{read})$, where $b \in \C B$ and $b\notin M_{l-1}$, but subsequently $b\in M_l$,
%\item computation of the form $\bar{c}=a\cdot b$ (corresponding to multiplication $\bar{A}_{ik}\cdot \bar{B}_{kj}$ into the entry $\bar{C}_{ij}$), 
%        $s_l=(\bar{c},a,b,\mathrm{compute})$, where $a\in \C A$, $b\in \C B$, and $a,b\in M_{l-1}$, while $\bar{c}\notin M_{l-1}$, 
%        but subsequently, $\bar{c}\in M_l$ (multiple partial sums of $\bar{C}_{ij}$ may not be in cache concurrently),
%\item computation of the form $\bar{c}=\bar{c}+a\cdot b$ (corresponding to multiplication $\bar{A}_{ik}\cdot \bar{B}_{kj}$ and its accumulation into the entry $\bar{C}_{ij}$), 
%        $s_l=(\bar{c},a,b,\mathrm{compute})$, where $a\in \C A$, $b\in \C B$, and $a,b,\bar{c}\in M_{l-1}$,
%\item computation of the form $c=c+\bar{c}$ (corresponding to symmetrization of $\C{\bar{C}}$ into $\C{C}$)
%        $s_l=(c,\bar{c},\mathrm{compute})$, where  $c,\bar{c}\in M_{l-1}$ and subsequently $\bar{c}\notin M_{l}$,
%\item copy of the form $c=\bar{c}$ (corresponding to symmetrization of $\C{\bar{C}}$ into $\C{C}$ or a simple set when symmetrization of $\C{\bar{C}}$ is not necessary, namely when $\C{\bar{C}}$ is a vector)
%        $s_l=(c,\bar{c},\mathrm{copy})$, where $\bar{c}\in M_{l-1}$ and subsequently $c\in M_l$ and $\bar{c}\notin M_l$,
%\item discard of values of $\C A$ from cache, $s_l=(a,\mathrm{discard})$, where $a \in \C A$ and $a \in \C M_{l-1}$, but subsequently $a\notin M_l$,
%\item discard of values of $\C B$ from cache, $s_l=(b,\mathrm{discard})$, where $b \in \C B$ and $b \in \C M_{l-1}$, but subsequently $b\notin M_l$,
%%\item discard of partial sums of $\C{\bar{C}}$ from cache, $s_l=(\bar{c},\mathrm{discard})$, where $\bar{c} \in \C M_{l-1}$, but subsequently $\bar{c} \notin M_l$,
%\item write/accumulate from cache to memory, $s_l=(c,\mathrm{write})$, where $c \in \C C$ and $c \in \C M_{l-1}$ but subsequently $c\notin M_l$.
%\end{itemize}
%%The `compute' operations  of the form $c=a+b$ and $c=c+a$, where $a,b,c$ are assumed to be disjoint,
%%add the value $c$ to the cache. In general, all operands of compute operations must be in 
%Each of the $\chchoose{n}{s}\chchoose{n}{t}\chchoose{n}{v}$ multiplications necessary for the direct evaluation algorithm must correspond to a `compute' operation in the schedule.
%Each of $\chchoose{n}{s}\chchoose{n}{t}\chchoose{n}{v} + \chchoose{n}{s}\chchoose{n}{t}$ additions must correspond to a `compute' operation
%or an accumulate (`write') operation in the schedule. All computed entries of $\C C$ (results of compute operations), must also be written or accumulated to the output,
%and output entries may not be overwritten. The `copy' operations are free as they do not correspond to any computation, but are simply a relabeling.
%We note that while the direct evaluation symmetric contraction algorithm must implicitly 
%compute the multiplications necessary to form the $\C{\bar{C}}$ intermediate, under our model this schedule forces accumulation to memory of the intermediates and multiplications directly  
%to the output $\C C$ itself (since the entries of $\C{\bar{C}}$ must be eventually accumulated there anyway).
%We measure the communication cost of the schedule as the number of `read' and `write' operations in $S$, therefore accumulating directly to $\C C$ is always more sensible
%than accumulating to some other intermediate. 
%%The communication cost of the `discard' operation $s_l\in S$, $s_l=(x,\mathrm{discard})$ is zero and it removes $x$ from $M_l$ ($x$ must be present in $M_{l-1}$).
%%The communication cost of a `read' operation $s_l\in S$, $s_l=(x,\mathrm{read})$ is one and it adds $x$ to $M_l$ ($x$ must not be present in $M_{l-1}$).
%%The communication cost of a `write' operation $s_l\in S$, $s_l=(x,\mathrm{write})$ is one and it removes $x$ from $M_l$ ($x$ must be present in $M_{l-1}$).
%The formulation of this schedule is strict in the sense that it precludes recomputation of contributions to $\C C$ as well as any other operations that 
%don't contribute directly to algorithmic progress.
%
%We now define a new schedule $\hat{S}$ from $S$, with cache store $\hat{M}_l$ after operation $s_l\in \hat{S}$, which computes matrix multiplication of two arbitrary (nonsymmetric) matrices
%$\C{\hat{C}} = \C{\hat{A}}  \C{\hat{B}}$, where the dimensions of $\C{\hat{A}}$ are $\chchoose{n}{s}$ by $\chchoose{n}{v}$ and the dimensions
%of $\C{\hat{B}}$ are $\chchoose{n}{v}$ by $\chchoose{n}{t}$. The new schedule $\hat{S}$ mimics $S$ by reading and discarding all symmetrically
%equivalent entries in $\C A$ and $\C B$, while computing and writing multiplications which contribute to an entry of $\C{\bar{C}}$ to the same destination in $\C{\hat{C}}$.
%We say that a pair of entries in $\bar{A}_{ij}, \bar{A}_{kl} \in \C A$ are {\it symmetrically equivalent} if they are folded from entries $\bar{A}_{ij}=A_\tpl{i}{s+v}$, $\bar{A}_{kl}=A_\tpl{j}{s+v}$
%and there exists a permutation $\pi$ such that $\tpl{i}{s+v}=\pi(\tpl{j}{s+v})$. There are sets of size up to $(s+v)!$ of symmetrically equivalent entries $\C A$, but only $(s+v)!/(s!v!)$ in $\C{\bar{A}}$,
%since the folded matrix $\C{\bar{A}}$ does not include entries that are symmetrically equivalent in permutation within $\tpl{j}{s}$ and within $\tpl{l}{v}$ for any entry $A_{\tpl{j}{s}\tpl{l}{v}}$.
%Similarly, for $\C B$, the folded matrix $\C{\bar{B}}$ contains sets of size up to $(v+t)!/(t!v!)$ of entries which are symmetrically equivalent due to the symmetry in $\C B$.
%%which is just the entry of $\C{\bar{C}}$ of which the intermediate is a contribution. 
%Formally, for the $i$th operation $s_l$ for $l=\inti{1}{|S|}$, we append the following operations to $\hat{S}$ (or ignore it if its not one of the below):
%\begin{itemize} 
%\item if $s_l=(a,\mathrm{read})$, where $a\in \C A$, we add up to $(s+v)!/(s!v!)$ read operations of all entries of $\C{\hat{A}}$ to $\hat{S}$ 
%      which have the same indices as those which are symmetrically equivalent to $a$ in the matrix $\C{\bar{A}}$ (there may be fewer than $(s+v)!/(s!v!)$ if the entry is on some diagonal in $\C A$),
%      thus for all `compute' operations for which $a$ can be an operand in $S$, we have loaded the corresponding entries in $\C{\hat{A}}$,
%\item if $s_l=(b,\mathrm{read})$, where $b\in \C B$, we add up to $(v+t)!/(t!v!)$ read operations of all entries of $\C{\hat{B}}$ to $\hat{S}$ which have the same indices as those which are symmetrically equivalent to $b$ in the matrix $\C{\bar{B}}$,
%      thus for all `compute' operations for which $b$ can be an operand in $S$, we have loaded the corresponding entries in $\C{\hat{B}}$,
%\item if $s_l=(\bar{c},a,b,\mathrm{compute})$ of the form $\bar{c}=a\cdot b$ or of the form $\bar{c}=\bar{c}+a\cdot b$ and corresponds to multiplication $\bar{A}_{ik}\cdot \bar{B}_{kj}$, we add a compute 
%        operation $\hat{c}=\hat{c} + \hat{A}_{ik}\cdot \hat{B}_{kj}$ to $\hat{S}$ where $\hat{c}$ is a partial sum to be accumulated into $\hat{C}_{ij}$, if there is already an existing $\hat{c}$ partial 
%        sum of $\hat{C}_{ij}$ is in $\hat{M}_{l-1}$ and add
%        operation $\hat{c}=\hat{A}_{ik}\cdot \hat{B}_{kj}$ to $\hat{S}$ if no partial sum of $\hat{C}_{ij}$ was in $\hat{M}_{l-1}$,
%%        operation $\hat{C}_{ij}=\hat{C}_{ij} + \hat{A}_{ik}\cdot \hat{B}_{kj}$ to $\hat{S}$ if $\hat{C}_{ij}$ is in $\hat{M}_{l-1}$ and add
%%        operation $\hat{C}_{ij}=\hat{A}_{ik}\cdot \hat{B}_{kj}$ to $\hat{S}$ if $\hat{C}_{ij}$ is not in $\hat{M}_{l-1}$ 
%%\item if $s_l=(c,a,b,\mathrm{compute})$ of the form $c=c+a\cdot b$ and corresponds to multiplication $\bar{C}_{ij}=\bar{A}_{ik}\cdot \bar{B}_{kj}$, we add a compute 
%%        operation $\hat{C}_{ij}=\hat{C}_{ij} + \hat{A}_{ik}\cdot \hat{B}_{kj}$ to $\hat{S}$ if $\hat{C}_{ij}$ is in $\hat{M}_{l-1}$ and add
%%        operation $\hat{C}_{ij}=\hat{A}_{ik}\cdot \hat{B}_{kj}$ to $\hat{S}$ if $\hat{C}_{ij}$ is not in $\hat{M}_{l-1}$ 
%\item if $s_l=(a,\mathrm{discard})$, where $a\in \C A$, we add up to $(s+v)!/(s!v!)$ discard operations of all entries of $\C{\hat{A}}$ to $\hat{S}$ which have the same indices as those which are symmetrically equivalent to $a$ in the matrix $\C{\bar{A}}$,
%\item if $s_l=(b,\mathrm{discard})$, where $b\in \C B$, we add up to $(v+t)!/(t!v!)$ discard operations of all entries of $\C{\hat{B}}$ to $\hat{S}$ which have the same indices as those which are symmetrically equivalent to $b$ in the matrix $\C{\bar{B}}$,
%\item if $s_l=(c,\mathrm{write})$, where $c \in \C C$, we add up to $(s+t)!/(s!t!)$ write or accumulate operations all contributions to $\C{\hat{C}}$ in $M_{l-1}$ which have the same indices as those which are symmetrically equivalent to the entry to which $c$ contributes in $\C{\hat{C}}$ (which discards these partial sums from $M_l$). 
%\end{itemize}
%The resulting schedule $\hat{S}$ computes the correct answer $\C{\hat{C}}$, as it performs the $\chchoose{n}{s}\chchoose{n}{v}\chchoose{n}{t}$ multiplications needed,
%as those must also be done to compute $\C{\bar{C}}$ by the direct evaluation symmetric contraction algorithm schedule. Further, it always has the needed operands to compute the multiplications,
%since whenever an entry $a\in \C{\bar{A}}$ or $b \in \C{\bar{B}}$ resides in $S$, all entries to which are symmetrically equivalent to $a$ or $b$ via the symmetry of $\C{A}$ and $\C{B}$ (for which
%$a$ or $b$ may act as operands in place of) are loaded from $\C{\hat{A}}$ or $\C{\hat{B}}$ by $\hat{S}$ and kept in memory until $a$ or $b$ is discarded by $S$.
%While the direct evaluation symmetric contraction schedule
%accumulates the partial sums of $\C{\bar{C}}$ to partial sums of $\C{C}$, prior to writing them to memory, the schedule $\hat{S}$ accumulates all the partial sums of $\C{\hat{C}}$ to memory whenever
%a partial sum of $\C{C}$ with a symmetrically equivalent entry is written by $S$.
%%accumulates the contribution to an entry with equivalent indices to $\C{\bar{C}}$ in
%%$\C{\hat{C}}$ (effectively explicitly forming the intermediate that $S$ may avoid forming by immediate symmetrization). 
%All contributions to $\C{\hat{C}}$, will %which we can label as a tuple $(i,j,k)$ will always
%be written or accumulated to memory (accumulated if another contribution has already been written to this entry), since they correspond to a partial sum of $\C{\bar{C}}$ of the same index, which
%must be accumulated or copied into an entry of $\C{C}$, which must subsequently be written, and for each operation that writes an entry of $\C{C}$ to memory, $\hat{S}$ writes to memory all
%entries of $\C{\hat{C}}$, that have the same index as any partial sum that could have been accumulated into this partial sum of $\C{C}$.
%% it is written
%%each time a contribution to $\C{C}$ is written or accumulated to memory in $S$,
%%$\hat{S}$ accumulates all contributions of $\C{\hat{C}}$ present in cache (whose multiplications were performed) corresponding to a the same tuple $(i,j,k)$ contribution to $\C{\bar{C}}$.
%
%Further, the cache size necessary to compute $\hat{S}$ is no more than 
%$r \cachesize=\max\lt(\frac{(s+v)!}{s!v!},\frac{(v+t)!}{t!v!},\frac{(s+t)!}{s!t!}\rt) \cachesize$, since for each entry of $\C A$ present in cache at any given point in $S$, 
%at most $(s+v)!/(s!v!)$ entries of $\hat{A}$ are present in $\hat{S}$, as up to this number of symmetrically equivalent entries are read and discarded, whenever the corresponding of $\C A$ is read or
%discarded. A similar argument for entries of $\C{\hat{B}}$ yields the factor of $\frac{(v+t)!}{t!v!}$. For partial sums of $\hat{c}\in \C{\hat{C}}$, we notice that whenever some partial sum is in $\hat{S}$ there
%must either by a partial sum of $\bar{c}\in \C{\bar{C}}$ with the same index as $\hat{c}$ or a partial sum of $c \in \C{C}$ to which $\bar{c}$ was copied or accumulated into and which corresponds to 
%an entry in $\C{C}$ to which $\hat{c}$ is symmetrized into.
%Since there at most $(s+t)!/(s!t!)$ entries (and partial sums of unique index) in $\C{\bar{C}}$ that are symmetrized into the same entry of $\C{C}$ and these are accumulated to memory (and therefore discarded),
%whenever the entry of $\C{C}$ is accumulated, there can be no more than $(s+t)!/(s!t!)$ different partial sums present in $\hat{S}$ for each partial sum present in $S$.
%% entries ever
%%existbe created in $\hat{S}$ for each entry of $\C{\bar{C}}$ that is created and copied or accumulated into a partial sum of $\C{C}$
%% in $S$, and whenever the latter is discarded, all of the former are too.
%The number of reads and writes in $\hat{S}$ is by a similar argument no greater than a factor of $r$ of those in $S$.
%Therefore, we've created a valid schedule for matrix multiplication of arbitrary matrices with cost no more than
%$\bwcost_\mathrm{MM}(n^s/s!,n^t/t!,n^v/v!,r \cachesize) \leq r \bwcost_\Psi (n,s,t,v,\cachesize)$.
%%The definition of such a matrix multiplication schedule is straight-forward, 
%%for each entry of $\C A$ or $\C B$ read by the symmetric contraction algorithm,
%%we consider the  $(s+v)!/(s!v!)$ equivalent entries of $\C A$ and 
%%the  $(v+t)!/(t!v!)$ equivalent entries of $\C B$ in the folded matrix representation,
%%and let the nonsymmetric matrix multiplication schedule read all of these 
%%(potentially non-equivalent) entries of nonsymmetric matrices $\C{\bar{A}}$ 
%%and $\C{\bar{B}}$. The nonsymmetric
%%schedule similarly mimics the behavior of the direct evaluation symmetric tensor contraction
%%algorithm with respect to keeping operands in cache (it keeps all the reflections
%%of each entry in cache). Since the direct evaluation symmetric tensor contraction
%%algorithm has to perform all
%%the $n^{s+v+t}/(s!t!v!)$ scalar multiplications, the nonsymmetric matrix multiplication
%%algorithm can do the same multiplications, and will always have the needed operands since the
%%symmetric tensor contraction algorithm does and all symmetrically equivalent entries
%%that it may take advantage of are explicitly read or kept by the nonsymmetric 
%%algorithm. The nonsymmetric algorithm ignores all the symmetrizations of $\C C$
%%entries done by the symmetric tensor contraction algorithm and writes back to memory
%%all $(s+t)/(s!t!)$ contributions to $\C{\bar{C}}$ (some which may be of value $0$) 
%%for each scalar contribution to $\C C$ performed by the symmetric tensor 
%%contraction algorithm. Its evident that this nonsymmetric matrix multiplication
%%algorithms needs no more than a factor of $r$ more memory than the symmetric
%%tensor contraction algorithm, and performs no more than a factor of $r$ more
%%communication. 
The computation cost of the schedule $\mathcal S$ is minimal (for the partially symmetric contraction) so long as we do not actually compute additions of elements with zero.
The communication cost of the schedule $\hat{\mathcal S}$ is a factor of $q$
%\[r=\max\lt({s+v\choose s},{v+t\choose t},{s+t \choose s}\rt),\]
greater than that of $\mathcal S$, since the three factors in the max defining $q$ correspond to the number of elements in each
set: $\mathring{A}_{\tpl{i}{s+v}}$, $\mathring{B}_{\tpl{i}{v+t}}$, and $\mathring{C}^{(g)}_{\tpl{i}{s+t}}$, respectively,
which are communicated whenever a corresponding element of $\C A$, $\C B$, or a partial sum of an element of $\C C$ is.
Similarly, the memory consumption of $\mathcal S$ is also greater by a factor of $q$.

Now, the tensor contraction,
\[\hat{C}_{\tpl js \tpl lt}=  \sum_{\tpl kv\in\enti 1nv} \hat{A}_{\tpl js\tpl kv}\cdot \hat{B}_{\tpl kv\tpl lt},\]
is equivalent to a matrix multiplication of tensors with dimensions $\chchoose ns\times \chchoose nv$ by $\chchoose nv \times \chchoose nt$
by the same argument as given after the definition of Algorithm~\ref{alg:systsy}.
%, except this time there is no symmetric equivalence between elements,
Since $\BH A$ and $\BH B$ can be arbitrary partially symmetric tensors and have the same number of unique entries as these matrices, this partially symmetric contraction
can be used to compute a matrix multiplication, and therefore cannot cost more than such a matrix multiplication,
%Therefore, the we can reduce the other way, from a matrix multiplication to this partially symmetric contraction, and
%assert that this partially symmetric contraction cannot be faster than the nonsymmetric matrix multiplication,
%which using the 
%Application of the lower bound in Theorem~\ref{thm:seq_comm_lwb_mm} yields
\begin{alignat*}{2}
\bwcost_\Psi(n,s,t,v,\cachesize)& \geq&& \frac{1}{q} \bwcost_\mathrm{MM}\lt(\chchoose ns,\chchoose nt,\chchoose nv,q \cachesize\rt).
%            & \geq && \frac{1}{r} \frac{2n^{s+v+t}}{s!t!v!\sqrt{q \cachesize}} \\
%            & = &&\frac{1}{r^{3/2}} \frac{2n^{s+v+t}}{s!t!v!\sqrt{\cachesize}} \\
%            & =&& \min\lt(\frac{s!v!}{(s+v)!},\frac{t!v!}{(v+t)!},\frac{s!t!}{(s+t)!}\rt)^{3/2} \\
%              & && \frac{2n^{s+v+t}}{s!t!v!\sqrt{\cachesize}}.
\end{alignat*}
Combining the above lower bound, with the trivial lower bound from reading the
inputs and writing outputs, we obtain the bounds stated in the theorem.
%\begin{alignat*}{2}
%\bwcost(n,s,t,v,\cachesize)  & \\
%\geq \max\Bigg[&\min\lt(\frac{s!v!}{(s+v)!},\frac{t!v!}{(v+t)!},\frac{s!t!}{(s+t)!}\rt)^{3/2} \frac{2n^{s+v+t}}{s!t!v!\sqrt{\cachesize}}, \\
%                   &\frac{n^{s+t}}{(s+t)!}+ \frac{n^{s+v}}{(s+v)!}+ \frac{n^{v+t}}{(v+t)!}\Bigg].
%\end{alignat*}
\end{proof}

\subsubsection{Horizontal communication lower bound}
\label{apx:par_comm_drct}

We now similarly prove the horizontal communication lower bound for parallel schedules given in Lemma~\ref{lem:comm_lowerb_syst_prl1} and restated below.
\begin{lemma}%\label{lem:comm_lowerb_syst_prl1}
Any load balanced schedule of $\systalg ABstv$
on $\Lambda(p,M)$ has horizontal communication cost, %a parallel machine with $p$ processors each with $M$ memory
%i.e. the number of words moved between the processors,
%under the assumptions that the work is balanced is %\fixme{Edgar}{make this precise} is
%(every processor does $O(F^\Upsilon(\varrho,n,s,t,v)/p)$ work)
%and that all elements have unit element size has the following lower bound,
$W_\Psi(n{,}s{,}t{,}v{,}p{,}M)$
\begin{align*}
=\Omega\lt(W_\mathrm{MM}\lt(\chchoose{n}{s},\chchoose{n}{t},\chchoose{n}{v},p,qM\rt)\rt),
\end{align*}
where $q=\max\lt({s+v\choose s},{v+t\choose t},{s+t \choose s}\rt)$.
\end{lemma}

\begin{proof}
Given any parallel schedule $\mathcal Q$ for $\systalg ABstv$, we can construct a schedule $\hat{\mathcal Q}$
that transforms $\mathcal Q$ to perform a partially symmetric contraction in almost the exact same fashion as done for the vertical communication cost lower bound.
The only difference is that the horizontal communication rather than vertical communication needs to be mimicked by
$\hat{\mathcal Q}$, which again satisfies all the dependencies. Further, each addition,
\[C^{(g)}_\tpl{i}{s+t}=C^{(f_1)}_\tpl{i}{s+t}+C^{(f_2)}_\tpl{i}{s+t},\]
in $\mathcal Q$ yields up to ${s+t \choose s}$ additions between elements of the sets 
$\mathring{C}^{(f_1)}_\tpl{i}{s+t}$ and $\mathring{C}^{(f_2)}_\tpl{i}{s+t}$ in $\hat{\mathcal Q}$.
In the sequential case, the total amount of work done by $\hat{\mathcal Q}$ was nevertheless minimal, so this did not matter, however,
in the parallel case it may make the work imbalanced. 
Nevertheless, the imbalance is a factor of at most ${s+t \choose s}$, which we assume is a constant, so the resulting schedule $\hat{\mathcal Q}$
is still asymptotically load balanced.

Therefore, the communication cost of $\mathcal Q$ cannot be less than a factor of $1/q$ multiplied by the cost of a matrix multiplication
of matrices with dimensions $\chchoose ns\times \chchoose nv$ and $\chchoose nv \times \chchoose nt$ and with a factor of $q$ more memory,
as the lemma states.
\end{proof}



==> nest_lb.tex <==


\begin{definition}
We say a matrix $\B A\in \mathbb{R}^{n_1\times n_2}$ is a $\sigma$-expander for some nondecreasing and positive function $\sigma \in \inti{1}{n_2} \to \mathbb{R}$, if $\forall k\in[1,n]$, any subset of $k$-columns of $\B A$, $\B{A^{(k)}}$ satisfies
\[\rank(\B{A^{(k)}})\geq \sigma(k).\]
\end{definition}

We observe that since the rank of any matrix cannot exceed the number of columns, any $\sigma$-expander matrix, also satisfy $\sigma(k)\leq k$.

The following Lemma shows that tensor products of two expander matrices result in an expander matrix. This Lemma leads from a known property of (Kronecker) tensor products, for any matrices $\B A$, $\B B$,
\[\rank(\B A\otimes \B B) = \rank(\B A)\rank(\B B).\]

\begin{lemma}
For any matrix $\B{A}\in \mathbb{R}^{n_1\times n_2}$ that is a $\sigma_A$-expander and any matrix $\B{B}\in \mathbb{R}^{m_1\times m_2}$ that is a $\sigma_B$-expander, $\B C = \B A \otimes \B B$ is a $\sigma_C$-expander where,
\[\sigma_C(k) = \min_{k_A\in\inti{1}{n_2},k_B\in \inti{1}{m_2}, k_Ak_B=k} (\sigma_A(k_A)\sigma_B(k_B)).\]
\end{lemma}
\begin{proof}
Let $\B{\mathcal{K}_A},\B{\mathcal{K}_B}$ be orthogonal matrices spanning the kernels of $\B{A}$ and $\B{B}$, respectively.
We can partition the kernel of $\B{C}$ into two possibly overlapping vector spaces, spanned by the orthogonal matrices
$\B{\mathcal{K}_1}$ and $\B{\mathcal{K}_2}$, respectively, where
\[\B{\mathcal{K}_1} = \B{\mathcal{K}_A} \otimes \B{I^{m_2\times m_2}} \quad\quad \mathrm{and} \quad\quad
  \B{\mathcal{K}_2} = \B{I^{n_2\times n_2}} \otimes \B{\mathcal{K}_B},\]
where each $\B{I^{y\times y}}$ represents a $y\times y$ identity matrix.

Now, for any $k\in\inti{1}{n_2m_2}$, consider a subset of $k$ columns $\B{C^{(k)}}$ of $\B C$, defined by $n_2m_2\times k$ projection matrix $\B P$ (which is a subset of $k$ columns of $\B{I^{n_2m_2\times n_2m_2}}$), so $\B{C^{(k)}}= \B C\B P$.
The kernel of $\B{C^{(k)}}$ is a projected subspace spanned by some subset of columns of the matrix ${\B P}^\mathsf{T}\B [\B{\mathcal{K}_1},\B{\mathcal{K}_2}]$, since
\[\B C\B P{\B P}^\mathsf{T} [\B{\mathcal{K}_1},\B{\mathcal{K}_2}] = \B C[\B{\mathcal{K}_1},\B{\mathcal{K}_2}] =0,\]
and since for any vector $\B v$, such that $\B{C^{(k)}}\B v=0$, we have $\B C ({\B P}\B v)=0$ (so $\B P\B v$ is in the span of $[\B{\mathcal{K}_1},\B{\mathcal{K}_2}]$ and consequently within the projected kernel subspace).
\end{proof}


==> par_comm_drct.tex <==

As in the sequential bounds, a parallel horizontal communication lower bound of the direct evaluation algorithm is again obtained by reduction from matrix multiplication. 
%but again from a smaller matrix multiplication than the nonsymmetric case. 
In this case, the reduction can cause some computation imbalance, but only by a constant factor as shown in the proof.
\begin{lemma}\label{lem:comm_lowerb_syst_prl1}
Any load balanced schedule of $\systalg ABstv$
on $\pararch{p}{M}$ has horizontal communication cost, %a parallel machine with $p$ processors each with $M$ memory
%i.e. the number of words moved between the processors,
%under the assumptions that the work is balanced is %\fixme{Edgar}{make this precise} is
%(every processor does $O(F^\Upsilon(\varrho,n,s,t,v)/p)$ work)
%and that all elements have unit element size has the following lower bound,
$W_\Psi(n{,}s{,}t{,}v{,}p{,}M)$
\begin{align*}
=\Omega\lt(W_\mathrm{MM}\lt(\chchoose{n}{s},\chchoose{n}{t},\chchoose{n}{v},p,qM\rt)\rt),
\end{align*}
where $q=\max\lt({s+v\choose s},{v+t\choose t},{s+t \choose s}\rt)$.
\end{lemma}
The proof of Lemma~\ref{lem:comm_lowerb_syst_prl1} follows that of the proof of Theorem~\ref{thm:comm_lowerb_strd}, constructing a matrix multiplication schedule from a schedule for $\systalg ABstv$ in the same fashion.
Therefore, we also give the proof of Lemma~\ref{lem:comm_lowerb_syst_prl1} in Appendix~\ref{apx:par_comm_drct}.

However, in the parallel case we derive an additional horizontal communication lower bound for cases when exactly one of $s,t,v$ is zero.
The additional bound is stronger than the bound obtained via the reduction from matrix multiplication when $s,t,v$ are all unequal (and one is zero).
In the sequential scenario, the communication cost of such cases is dominated by reading the inputs from memory to cache or writing the output to memory.
In the parallel scenario, the largest tensor can be kept in place, so communication of the second-largest tensor must be considered.
When $v=0$, the new communication lower bound then arises as a consequence of symmetrization needed to compute $\B C$. 
When $s=0$ or $t=0$, this bound is a consequence of the assumption that each unique elements of the largest the symmetric operand is stored on a unique processor.
%are not stored redundantly (i.e. each unique entry exists on a unique processor).
%to our assumption that only unique entries of the tensors are stored at the beginning of execution and each entry
%of the output is only computed once.
This assumption corresponds to a `packed' distributed layout~\cite{SMHSD_JPDC_2014}. Therefore, using an `unpacked' layout where the tensor operands are stored as if they were nonsymmetric.
% by storing each symmetrically equivalent entry in the tensor on different processors. 
%  that each unique entry is stored on a unique processor (e.g. storing all entries of the symmetric operands) 
would make it possible to have asymptotically lower communication costs in cases when either $s$ or $t$ is zero and $v\neq s$ as well as $v\neq t$.
%From a practical perspective, this implies that packed distributed storage of tensors (which minimizes memory)~\cite{SMHSD_JPDC_2014} 
%has its disadvantages for certain contractions.
\begin{lemma}\label{lem:comm_lowerb_syst_prl2}
When exactly one of $s,t,v$ is zero, any load balanced schedule of $\systalg ABstv$ on $\pararch{p}{M}$ has horizontal communication cost, %a parallel machine with $p$ processors each with $M$ memory
%i.e. the number of words moved between the processors,
%under the assumptions that the work is balanced is %\fixme{Edgar}{make this precise} is
%(every processor does $O(F^\Upsilon(\varrho,n,s,t,v)/p)$ work)
%and that all elements have unit element size has the following lower bound,
$W_\Psi(n{,}s{,}t{,}v{,}p{,}M)$
%\begin{align*}
%=\Omega\lt(W_\mathrm{MM}\lt(\chchoose{n}{s},\chchoose{n}{t},\chchoose{n}{v},p,qM\rt)\rt),
%\end{align*}
%where $q=\max\lt({s+v\choose s},{v+t\choose t},{s+t \choose s}\rt)$.
%Further, 
%such cases correspond to the third scenario is Theorem~\ref{thm:par_comm_lwb_mm}, where the 
%smallest matrix (with dimensions $x$ and $y$) is communicated.
\[W_\Psi(n,s,t,v,p,M) = \Omega\lt((n^\omega/p)^{\max(s,t,v)/\omega}\rt).\]
%\fixed{Edgar}{The above is only true for $m,n,k\gg 1$, do the other cases.}
%\fixed{Edgar}{Prove this with constants using Loomis-Whitney. Nah}
\end{lemma}
\begin{proof}
%Given any parallel schedule $\mathcal Q$ for $\systalg ABstv$, we can construct a schedule $\hat{\mathcal Q}$
%that transforms $\mathcal Q$ to perform a partially symmetric contraction in almost the exact same fashion as done for the vertical communication cost lower bound.
%\fixme{Edgar}{This is now in Appendix, so below is not very comprehensible.}
%The only difference is that the horizontal communication rather than vertical communication needs to be mimicked by
%$\hat{\mathcal Q}$, which again satisfies all the dependencies. Further, each addition,
%\[C^{(g)}_\tpl{i}{s+t}=C^{(f_1)}_\tpl{i}{s+t}+C^{(f_2)}_\tpl{i}{s+t},\]
%in $\mathcal Q$ yields up to ${s+t \choose s}$ additions between elements of the sets 
%$\mathring{C}^{(f_1)}_\tpl{i}{s+t}$ and $\mathring{C}^{(f_2)}_\tpl{i}{s+t}$ in $\hat{\mathcal Q}$.
%In the sequential case, the total amount of work done by $\hat{\mathcal Q}$ was nevertheless minimal, so this did not matter, however,
%in the parallel case it may make the work imbalanced. 
%Nevertheless, the imbalance is a factor of at most ${s+t \choose s}$, which we assume is a constant, so the resulting schedule $\hat{\mathcal Q}$
%is still asymptotically load balanced.
%
%Therefore, the communication cost of $\mathcal Q$ cannot be less than a factor of $1/q$ multiplied by the cost of a matrix multiplication
%of matrices with dimensions $\chchoose ns\times \chchoose nv$ and $\chchoose nv \times \chchoose nt$ and with a factor of $q$ more memory,
%as the theorem states.
%
%We now prove the second bound, which applies when exactly one of $s,t,v=0$. 
%\fixed{Edgar}{proof sketch start}
Consider all $\bar{F}={\chchoose ns}{\chchoose nt}{\chchoose nv}$ multiplications in \eqref{eq:symctr}, 
% in which $\tpl js$, $\tpl lt$, and $\tpl kv$ contain no repeated indices.
%Since the total number of multiplications needed by $\systalg ABstv$ ,
some processor $p_i$ must perform at least $F=\bar{F}/p\geq\frac{n^\omega}{s!t!v!p}$ such multiplication operations. %, but computes only $K=\frac{n^\omega}{(s+t)!p}$ elements of $\C C$.

Without loss of generality assume $v=0$ and $s\geq t$. The other cases may be proven similarly as we outline below.
Consider the largest tensor, in this case $\C C$, each entry of $\C C$ requires the addition of $\frac{(s+t)!}{s!t!}$ results of multiplications.
%(each entry of an operand participates in a corresponding number of multiplications).
Now, one of the following two cases holds,
\begin{enumerate}
%It must be the case that either $F/2$ flops done by this processor contribute to his the entries of $\C C$ it outputs, or $F/2$ of the flops contribute to other entries of $\C C$.
\item at least $F/2$ of the multiplications done by processor $p_i$ contribute to entries of $\C C$ which a processor other than $p_i$ outputs:
  these must contribute to at least $\frac{s!t!}{(s+t)!}F/2$ partial summations to entries of $\C C$, so at least $\frac{s!t!}{(s+t)!}F/2=\Omega(n^\omega/p)$,
  communication is necessary, which is stronger than the desired bound.
\item at least $F/2$ of the multiplications done by processor $p_i$ contribute to the entries of $\C C$ which $p_i$ outputs: 
  there are at least $K\defeq \frac{s!t!}{(s+t)!}F/2=\Omega(n^\omega/p)$ such entries.
\end{enumerate}
Since in the first case the desired bound is obtained immediately, we now focus on the second case, where $K$ of the multiplications processor $p_i$ computes contribute to entries of $\C C$ which $p_i$ outputs.
We again consider two cases, one of which must hold,
\begin{enumerate}
\item for at least $K/2$ entries of $\C C$ which $p_i$ outputs, $p_i$ receives at least one partial sum (a single or more accumulated multiplications) from some other processor:
      the processor must receive at least $K/2=\Omega(n^\omega/p)$ entries/partial-sums, which is stronger than the desired bound.
\item for at least $K/2$ entries of $\C C$ which $p_i$ outputs, $p_i$ computes all the multiplications.
\end{enumerate}
Again, the first case yields the bound immediately, therefore, we focus on the second case, where $p_i$ computes 
all multiplications necessary for $K/2=\Omega(n^\omega/p)$ entries of $\C C$.
Let this set of multiplications correspond to all entries $C_\tpl{i}{s+t}$ for $\tpl i{s+t}\in V\subseteq \enti 1n{s+t}$.
Computation of the $\B C$ entries given by this index set require the operands $\B A_{\tpl js}$ for all $\tpl js\in L_\mathrm{A}$, where
\[L_\mathrm{A}=\{\tpl js : \tpl js\in \prj s(\tpl{i}{s+t}), \tpl{i}{s+t}\in V\}\]
(keeping in mind that $\tpl{k}{v}$ does not exist since $v=0$).
We obtain a lower bound on the number of $\C A$ entries $|L_\mathrm{A}|$ needed to perform these multiplications by application of Lemma~\ref{thm:tlw} with $m=\omega=s+t$ and $r=s$, in particular,
\[|L_\mathrm{A}|\leq |V|^{s/\omega}=\Omega\lt((n^\omega/p)^{s/\omega}\rt).\]
This is asymptotically greater than the $\Theta(n^s/p)$ of entries of $\C A$ any processor can own by the load balanced schedule assumption, so most of these
entries must be obtained by communication, yielding the communication lower bound for the case $v=0$ and $s\geq t$,
\[W_\Psi(n,s,t,v,p,M) = \Omega\lt((n^\omega/p)^{s/\omega}\rt).\]

When $v=0$ and $t>s$, we can obtain a stronger bound with an exponent $t/\omega$, by considering the $\B B$ operands rather than the $\C A$ operands to $\C C$.
When $s=0$ or $t=0$ rather than $v=0$, we can first assert by a similar argument that $p_i$ must compute $F/2$ multiplications with at least $K=\frac{v!t!}{(v+t)!}F/2$ entries of $\C B$ (when $s=0$) 
or with at least $K=\frac{s!v!}{(s+v)!}F/2$ entries of $\C A$ (when $t=0$), which it starts with initially (otherwise it must receive enough other operands to prove the bound).
Then, rather than obtaining a lower bound of $K/2$ on the number of entries of $\C C$ some $p_i$ computes all the multiplications for, we would instead obtain a lower
bound on the number of entries of $\C B$ (when $s=0$) or $\C A$ (when $t=0$) for which $p_i$ computes all the multiplications each of these entries is an operand of 
(otherwise the processor must communicate at least $K/2$ operands). 
This last step is possible as a result of the assumption that each unique operand tensor entry is an input to a unique processor.
Lastly, knowing that $p_i$ computes all multiplications with $K/2$ of entries of the largest tensor (of order $\omega$), we would use Lemma~\ref{thm:tlw} to assert that the number of entries
of the second largest tensor (of order $\max(s,t,v)$) required for these multiplications is $(K/2)^{\max(s,t,v)/\omega}$.
Having covered all the orderings of the magnitudes of $s,t,v$ when one of them is zero, we have now shown the desired bound,
\[W_\Psi(n,s,t,v,p,M) = \Omega\lt((n^\omega/p)^{\max(s,t,v)/\omega}\rt).\]
\end{proof}
%The memory dependent lower bound was proven by~\cite{irony_mm_lb04} and the memory-independent lower bound previously by~\cite{aggarwal1989communication}.
%\begin{proof}
%The upper bound on the cost may be attained by 
%%the classical algorithm that computes matrix multiplication
%%block-by-block with blocks of each matrix of dimension $\sqrt{\cachesize/3}$.
%a 3D blocking
%of the matrix multiplication algorithm (first proposed and analyzed 
%by Berntsen~\cite{berntsen1989communication} and Aggarwal et al.~\cite{aggarwal1989communication}).
%
%We note that in practice, the ordering of elements in which the matrix is laid out in memory
%may present non-trivial overheads if the desired matrix element ordering is different.
%This challenge is amplified in the case when the tensor contraction is done on a distributed-memory system.

%\fixed{}{Cite \cite{greygeneral2010} and/or Snir, and this will probably need to be asymptotic.}

%\end{proof}

We now combine the above two lemmas to obtain the full lower bound for $\systalg ABstv$.
\begin{theorem}\label{thm:comm_lowerb_syst_prl}
Any load balanced schedule of $\systalg ABstv$
on $\pararch{p}{M}$ has horizontal communication cost, %a parallel machine with $p$ processors each with $M$ memory
%i.e. the number of words moved between the processors,
%under the assumptions that the work is balanced is %\fixme{Edgar}{make this precise} is
%(every processor does $O(F^\Upsilon(\varrho,n,s,t,v)/p)$ work)
%and that all elements have unit element size has the following lower bound,
$W_\Psi(n{,}s{,}t{,}v{,}p{,}M)$
\begin{align*}
=\Omega\lt(W_\mathrm{MM}\lt(\chchoose{n}{s},\chchoose{n}{t},\chchoose{n}{v},p,qM\rt)\rt),
\end{align*}
where $q=\max\lt({s+v\choose s},{v+t\choose t},{s+t \choose s}\rt)$.
Further, when exactly one of $s,t,v$ is zero, 
%such cases correspond to the third scenario is Theorem~\ref{thm:par_comm_lwb_mm}, where the 
%smallest matrix (with dimensions $x$ and $y$) is communicated.
\[W_\Psi(n,s,t,v,p,M) = \Omega\lt((n^\omega/p)^{\max(s,t,v)/\omega}\rt).\]
\end{theorem}
\begin{proof}
Theorem~\ref{thm:comm_lowerb_syst_prl} is trivially obtained by combining Lemma~\ref{lem:comm_lowerb_syst_prl1} and Lemma~\ref{lem:comm_lowerb_syst_prl2}.
\end{proof}



==> par_comm_prsv.tex <==

%The extension of these communication results to the parallel case is straight-forward
%since the computation of each scalar multiplication in the algorithm may be done in parallel,
%as with matrix multiplication. We state a memory-independent parallel communication lower bound
%in Theorem~\ref{thm:par_comm_lowerb}, whose proof demonstrates that the dependency graph of
%$\syfsalg ABstv$
%\fixme{Edgar}{This used to be a for loop alg.}
%%$\Phi^{(s,t,v)}$ (computed as Algorithm~\ref{alg:Znorm}) 
%is structurally an  \\
%\hlattice{\omega}{\kappa} by the definition in Chapter 3 of~\cite{ES_dissertation_2014}.

We now derive a lower bound on the horizontal communication cost of any parallel schedule for the symmetry preserving
algorithm, considering only cases when at least two of $s,t,v$ are nonzero (if two are zero, then $\syfsalg ABstv \equiv \systalg ABstv$). %, so this case does not require additional analysis.
As in the sequential case, we assume that partial sums are not reused to compute different operand elements in \eqref{eq:fschatZ} and that partial sums are also not reused to compute
contributions of $\BH Z$ to different elements of $\B Z$ in \eqref{eq:fscZ}.
%However, in this case it is more consequential: 
When $s,t,v>0$, by the same arguments as in the sequential case the reuse partial sums can only be useful when $s,t,v\geq 2$. 
However, when exactly one of $s,t,v$ is zero, the parallel cost is not dominated
by communicating in the largest tensor as in the sequential case, but rather with the communication cost associated with the second largest tensor,
so the reuse partial sums could potentially be useful when the two of $s,t,v$ are greater or equal to two and the third is zero.
Such cases can arise in coupled-cluster contractions~\cite{Bartlett:1981:ARPC:CC}.
\begin{theorem}\label{thm:par_comm_lowerb}
Any load balanced schedule of $\syfsalg ABstv$ on $\pararch{p}{M}$ has horizontal communication cost:
%$\syfsalg ABstv$ %$Phi_\odot^{(s,t,v)}(\C A,\C B)$ 
%on a homogeneous machine with $p$ processors each with local memory $M$
%is 
\begin{enumerate}
\item when $s,t,v\geq 1$,
  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{\kappa/\omega}\rt),\]
  where $\kappa \defeq \max(s+v,v+t,s+t)$,
\item when exactly one of $s,t,v$ is zero,
  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{\max(s,t,v)/\omega}\rt),\]
%\item \fixed{Edgar}{When two of $s,t,v$ are zero, I don't really care since $\Psi=\Phi$.}
\end{enumerate}
under the assumption that partial sums are not reused to compute different operand elements in \eqref{eq:fschatZ} and that partial sums are also not reused to compute 
contributions of $\BH Z$ to different elements of $\B Z$ in \eqref{eq:fscZ}.
\begin{align*}
\end{align*}
\fixme{Edgar}{Memory-dependent bound}
\end{theorem}
\begin{proof}
Consider the $\chchoose n\omega$ multiplications in \eqref{eq:fschatZ}, 
%where $\tpl{i}{\omega}$ 
%has no repeated indices.
some processor $p_i$ must perform at least $\chchoose n\omega/p$ of these multiplications,
computing $\hat{Z}_\tpl i\omega$ for each $\tpl i\omega$ in $\bar{V}$ where $\bar{V}\subseteq \enti 1n\omega$.
We now count the number of dependencies i.e. elements of $\B A$ and $\B B$ needed by any set of 
such multiplications, using the assumption that partial summations of these operands are
not reused for multiple elements of $\BH Z$. 
We also count the number of elements of $\B Z$ that are dependent on these multiplications,
again using an analogous assumption that partial summations of multiplications 
contributing to different elements of $\B Z$ are not reused.
These assumptions imply that for any operand or result of $\BH Z$, 
it never helps to communicate a partial sum, as a unique one is needed for each element of $\BH Z$. 
As a result, if for $|\bar{V}|/2$ of the multiplications $p_i$ computes, partial summations are
either of the $\B A$ or the $\B B$ operand are received or the computed element of $\BH Z$ is sent, 
we immediately get a communication cost of $\Omega(n^\omega/p)$, which is higher than the desired 
lower bounds. 
Therefore, there is a subset of the elements of $\BH Z$ with indices $V\subseteq \bar{V}$ of size
$|V|\geq |\bar{V}|/2$, for which the operands are either received or stored initially and for which
the element of $\BH Z$ is accumulated to a partial sum for each element of $\B Z$ to which
it contributes (otherwise this element of $\BH Z$ would have had to be communicated).

Having ruled out the use of partial summations, we can now cleanly derive lower bounds for the communication
due to each of the operands and the result.
%\begin{enumerate}
%\item 

{\bf Data Received:} The operands to the set of multiplications done by $p_i$ include all $\C A_{\tpl j{s+v}}$ for $\tpl j{s+v}\in L_\mathrm{A}$, where
  \[L_\mathrm{A}=\{\tpl{j}{s+v} : \tpl{j}{s+v}\in \prj{s+v}(\tpl{i}{\omega}),\tpl{i}{\omega}\in V\}.\]
    We can obtain a lower bound on the size of $L_\mathrm{A}$ by finding the number of unique indices
    $\tpl{j}{s+v}$ given by Lemma~\ref{thm:tlw} with $m=\omega$ and $r=s+v$,
  \[|L_\mathrm{A}| = |V|^{(s+v)/\omega} = \Omega\lt((n^\omega/p)^{(s+v)/\omega}\rt).\]
    When $t>0$, this is asymptotically larger than the $\Theta\lt(\frac{n^{s+v}}p\rt)$ elements of $\B A$, $p_i$ can
    own initially by the load balance assumption, so the number of elements of $\B A$ received by $p_i$ when $t>0$ is
  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{(s+v)/\omega}\rt).\]
    We can apply the same argument to the other operand $\B B$ and assert that when $s>0$,
  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{(v+t)/\omega}\rt).\]
%\item The different operands of $\C B$ to the set of multiplications done by $p_i$ are
%  \[L_\mathrm{B}=\{B_\tpl{l}{v+t} : \tpl{l}{v+t}\in \chi(\tpl{i}{\omega}),\tpl{i}{\omega}\in V\}.\]
%    We can obtain a lower bound on the size of $L_\mathrm{B}$ by finding the number of unique indices
%    $\tpl{l}{v+t}$ given by Lemma~\ref{thm:tlw} with $m=\omega$ and $r=v+t$,
%  \[|L_\mathrm{B}| = |V|^{(v+t)/\omega} = \Omega\lt((n^\omega/p)^{(v+t)/\omega}\rt).\]
%    When $s>0$, this is asymptotically larger than the $\Theta\lt(\frac{n^{v+t}}p\rt)$ elements of $\B A$, $p_i$ can
%    own initially by the load balance assumption, so the number of elements of $\B B$ received by $p_i$ when $s>0$ is
%  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{(v+t)/\omega}\rt).\]
%\item 

{\bf Data Sent:} The elements of $\C Z$ to which the set of multiplications done by $p_i$ contribute (in \eqref{eq:fscZacc}) are $Z_\tpl{h}{s+t}$ for all $\tpl{h}{s+t}\in L_\mathrm{Z}$, where
  \[L_\mathrm{Z}=\{\tpl{h}{s+t} : \tpl{h}{s+t}\in \prj{s+t}(\tpl{i}{\omega}),\tpl{i}{\omega}\in V\}.\]
    We can obtain a lower bound on the size of $L_\mathrm{Z}$ by finding the number of unique indices
    $\tpl{h}{s+t}$ given by Lemma~\ref{thm:tlw} with $m=\omega$ and $r=s+t$,
  \[|L_\mathrm{Z}| = |V|^{(s+t)/\omega} = \Omega\lt((n^\omega/p)^{(s+t)/\omega}\rt).\]
    When $v>0$, this is asymptotically larger than the $\Theta\lt(\frac{n^{s+t}}p\rt)$ elements of $\B Z$, $p_i$ can
    output by the load balance assumption, so the number of partial summations (multiplications or sums of multiplications contributing to a given element $Z_\tpl{h}{s+t}$) when $v>0$ is
  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{(s+t)/\omega}\rt).\]
%\end{enumerate}

Combining the data sent and data received lower bounds, we notice that when $s,t,v\geq 1$, all three of the above lower bounds apply and we get the
best bound by considering the largest tensor, which is of order $\kappa=\max(s+v,v+t,s+t)$ and yields the lower bound,
  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{\kappa/\omega}\rt).\]
When exactly one of $s,t,v$ is zero, we have no lower bound associated with the largest tensor (of order $\omega$),
but we have a lower bound associated with the second largest tensor, which is of order $\max(s,t,v)$,
  \[W_\Phi(n,s,t,v,p)= \Omega\lt((n^\omega/p)^{\max(s,t,v)/\omega}\rt).\]
%\[V = \{Z_\tpl i\omega : 
%\sum_{\tpl{j}{ s+v } \in \chi( \tpl{i}{\omega})} A_{\tpl{j}{ s+v }}\bigg) \cdot
%      \bigg(\sum_{\tpl{l}{ t+v } \in \chi( \tpl{i}{\omega})} B_{\tpl{l}{ t+v }}
%\fixme{Edgar}{prove case 2, check case 1 below.}
%Consider any dependency graph $G_\Phi=(V_\Phi,E_\Phi)$ 
%that computes $\syfsalg ABstv$.
%\fixme{Edgar}{This used to be a for loop alg.}
%%Algorithm~\ref{alg:Znorm}.
%It must compute all multiplications $\hat{Z}_\tpl{i}{\omega}$ for all ordered $\tpl{i}{\omega}$. 
%Each $\hat{Z}_\tpl{i}{\omega}$ is a dependent on all $A_\tpl{j}{s+v}$ where 
%$\tpl{j}{s+v}\in \tpl{i}{\omega}$ and on all $B_\tpl{l}{t+v}$ where $\tpl{l}{t+v} \in \tpl{i}{\omega}$,
%and contributes to the sum forming (is a dependency of) $Z_\tpl{j}{s+t}$ ($C_\tpl{j}{s+t}$) for all
%$\tpl{j}{s+t}\in \tpl{i}{\omega}$. We can therefore define a parent \\
%\hlattice{\omega}{\kappa}
%of breadth $n$ (as defined in Chapter 3 of~\cite{ES_dissertation_2014}) $H_\Phi=(V_\Phi^H,E^H_\Phi)$ where
%the vertices contain all entries $\C{\hat{Z}}_\tpl{i}{\omega} \in V_\Phi^H$ with
%$i_1 <\cdots <i_\omega$. Each hyperedge $e_\tpl{j}{\kappa} \in E^H_\Phi$ corresponds to
%the highest order projection
%(if $s+v$ largest then $\C A$, otherwise if $v+t$ largest then $\C B$, and otherwise if $s+t$
%is largest then $\C C$) and contains $e_\tpl{j}{\kappa}= \{\C{\hat{Z}}_\tpl{i}{\omega} \in V_\Phi^H : \tpl{j}{\kappa}\subset \tpl{i}{\omega}\}$. 
%These hyperedges are edge disjoint connected partitions, since each 
%corresponds either to all dependents of an operand tensor entry or to all dependencies of an output entry
%$Z_\tpl{j}{s+t}$, which must be combined via some reduction tree (the intermediate sums in
%the reduction tree are ignored in a parent hypergraph as in Chapter 5 of~\cite{ES_dissertation_2014}).
%Since we assume the computation is load balanced and $V^H_\Phi$ contains $\Theta(n^\omega)$ vertices,
%some processor must compute no more than $\lfloor |V^H_\Phi|/4\rfloor $ 
%vertices and at least $\lfloor |V^H_\Phi|/p\rfloor$. By 
%Theorem 3.3.1 in~\cite{ES_dissertation_2014}, the minimum \hcut{p}{4} of $H_\Phi$ is of size
%$\epsilon_p(H_\Phi)=\Omega(n^{\kappa}/p^{\kappa/\omega})$.
%Further by Theorem 3.2.2 in~\cite{ES_dissertation_2014}, since $H_\Phi$ is a parent hypergraph of 
%any dependency graph $G_\Phi$ and has degree at most ${\omega \choose \kappa}$ the
%minimum \vsep{p}{4} of any $G_\Phi$ is of size at least 
%$$\csexp{p}{4}{G_\Phi(n,s,t,v)}=\Omega(n^{\kappa}/p^{\kappa/\omega}).$$
%Since any communicated set is a \vsep{p}{4} of $G_\Phi$ (by definition in Chapter 3 of~\cite{ES_dissertation_2014}),
%the lower bound on separator size is also a lower bound on communication cost for any load-balanced
%execution of $\Phi^{(s,t,v)}$,
%  $$W^\Phi(n,s,t,v,p)= \Omega\left(\frac{n^{\kappa}}{p^{\kappa/\omega}}\right).$$
\end{proof}

%

%Overall this communication cost does not constitute a non-trivial 
%improvement over the standard algorithm, except when $\omega$ is quite large.
%However, for certain applications, the algorithm can be nested in a way that yields
%the same communication cost improvement as the reduction in the number of 
%multiplications with respect to the standard algorithm, namely $\omega!/(s!t!v!)$,
%which is a substantial improvement. We consider these in the next section.



==> seq_comm_drct.tex <==



==> seq_comm_prsv.tex <==
%We proceed to quantify the communication cost of the algorithm by specifying a lower and upper bound on the cost
%of a communication-optimal schedule.
We now derive a communication lower bound for Algorithm~\ref{alg:syfs} ($\syfsalg ABstv$). 
The proof is based on considering contiguous chunks of multiplications in \eqref{eq:fscmul} computed by any given schedule and using Lemma~\ref{thm:tlw} to demonstrate that each chunk requires communication as it cannot be done using exclusively cache-resident elements.
Unlike the matrix multiplication case, for the symmetry preserving algorithm it suffices to consider only the communication of the elements of (the largest) one of $\B{A}$, $\B{B}$, or $\B{Z}$.

Our proof assumes that no partial sums are reused to compute different entries of $\B{\hat{A}}$ \eqref{eq:fscAacc} and similarly for $\B{\hat{B}}$ \eqref{eq:fscBacc}, nor to compute $\B{Z}$ from $\B{\hat{Z}}$ in \eqref{eq:fscZacc}.
%partial sums are not reused to compute different operand elements in \eqref{eq:fschatZ} and that partial sums are also not reused to compute
%contributions of $\BH Z$ to different elements of $\B Z$ in \eqref{eq:fscZ}.
The reuse of such partial sums would change the number of operations as well as the dependency graph of the algorithm.
%This assumption is not needed when $v\leq s,t$, as in that case we ignore the operands (instead we consider contributions to $\B Z$).
We also argue that this assumption cannot have a significant effect in most use-cases.
In particular, such partial sums cannot help when $s=0$ or $t=0$ or $v=0$, since in these cases the lower bound is dominated by reading in the inputs or writing the outputs.
Additionally no shared partial sums exist when $\min(s,t,v)=1$, since the operands/results of the largest tensor (the only one the proof considers) may share only one summand/target in the summation with any other operand/result.
Therefore, this assumption is only significant when $s,t,v\geq 2$; we are not aware of applications for such cases.
\begin{theorem}\label{thm:comm_lowerb}\label{thm:comm_upperb}
Let $\kappa \defeq \max(s+v,v+t,s+t)$.
Any schedule of $\syfsalg ABstv$ on $\seqarch{\cs}$ has vertical communication cost,
%given a cache of size $\cachesize$ is 
\begin{align*}
%&\frac{n^\omega/\omega!}{(M/3)^{\omega/max(s+v,v+t,s+t)-1}}\cdot
%                        \lt[{\omega\choose t} 
%                            +{\omega\choose s} 
%                            +{\omega\choose v} \rt] + \frac{2n^{s+v}}{(s+v)!}+ \frac{2n^{v+t}}{(v+t)!} + \frac{2n^{s+t}}{(s+t)!} +
%                            O(n^{\omega-1}) \\
%
\bwcost_\Phi(n,s,t,v,\cachesize) \geq   \max\Bigg(&\left\lfloor\chchoose{n}{\omega}/(2\cachesize)^{\omega/\kappa}\right\rfloor \cachesize, 
                                    \frac{n^{s+t}}{(s+t)!}+ \frac{n^{s+v}}{(s+v)!}+ \frac{n^{v+t}}{(v+t)!}\Bigg). 
%  &         \leq    \bwcost^\Phi(n,s,t,v,\cachesize)\leq
%  \frac{n^\omega \cdot \big[{\omega \choose s}+{\omega \choose t} + {\omega \choose v}\big]^{1/\max(s+v,v+t,s+t)}}{\omega!\cdot \cachesize^{-1+\omega/\max(s+v,v+t,s+t)}}  + O(n^{s+t} + n^{s+v} + n^{v+t} + n^{\omega-1}),
\end{align*}
%%that partial sums are not reused to compute the summations needed for each operand in \eqref{eq:fschatZ}.
%under the assumption that partial sums are not reused to compute different operand elements in \eqref{eq:fschatZ} and that partial sums are also not reused to compute 
%contributions of $\BH Z$ to different elements of $\B Z$ in \eqref{eq:fscZ}.
%%assuming that all elements of $\C A$, $\C B$, and $\C C$ are of unit size.
\end{theorem}
\begin{proof}
%We give the proof for these lower and upper bounds in the Appendix (Section~\ref{sec:apx:comm}).
%The upper bound proof relies on a schedule that blocks the multiplications (tensor $\C{\hat{Z}}$) 
%symmetrically so that each block, along with its dependencies and outputs fit into cache.
%The lower bound proof relies primarily on more general theory of communication
%lower bounds for nested-loop computations~\cite{christ2013communication}.
%\renewcommand{\qedsymbol}{}


%{\bf Upper bound:}
%An upper bound on the communication cost of the algorithm
%may be obtained by providing a suitable execution schedule.
%Consider the following schedule, parameterized by $b$, which will be picked so that $b\ll n$, and where we assume $b$ divides into $n$ (otherwise the algorithm
%can be executed for a problem of size $n + (n\bmod b)$ padded with zeros, with no greater asymptotic cost since $b\ll n$). %, $k_t$, and $k_v$.
%We define a tensor $\C{\tilde{A}}$ whose elements are blocks of $\C{A}$ of order $s+v$ and with dimension $b$.
%%as $\C{\tilde{A}}$, such that $\C{\tilde{A}}$ is a tensor each element of which is a block of $\C A$ of order $s+v$, with
%%each dimension equal to $b$. 
%Each dimension of the tensor $\C{\tilde{A}}$ itself is $n/b$. Its elements are defined as follows $\forall \tpl{I}{s+v}\in \inti{0}{n/b-1}^{s+v}$,
%$$
%\tilde{A}^{\tpl{I}{s+v}}=\{ A_{\tpl{i}{s+v}} \ | \ 
%\ \forall \  \tpl{i}{s+v} = (b\cdot \tpl{I}{s+v} + \tpl{\hat{i}}{s+v}),  \tpl{\hat{i}}{s+v} \in \inti{1}{b}^{s+v}\}
%$$
%Similarly, we define
%blocked versions of $\C{B}$ and $\C{\hat{Z}}$ (where $\C{\hat{Z}}$ is as before the tensor of multiplications needed to compute $\C Z$) as
%\begin{alignat*}{4}
%\forall \tpl{I}{v+t}\in \inti{0}{n/b-1}^{v+t},& \\ 
%\tilde{B}^{\tpl{I}{v+t}}=&\{ B_{\tpl{i}{v+t}} \ | \ 
%\ \forall \  \tpl{i}{v+t} &&= (b\cdot \tpl{I}{v+t} + \tpl{\hat{i}}{v+t}), && \tpl{\hat{i}}{v+t} \in \inti{1}{b}^{v+t}\}, \\
%\forall \tpl{I}{\omega}\in \inti{0}{n/b-1}^{\omega},& \\\ \ 
%\tilde{Z}^{\tpl{I}{\omega}}=&\{ \hat{Z}_{\tpl{i}{\omega}} \ | \ 
%\ \forall \  \tpl{i}{\omega} &&= (b\cdot \tpl{I}{\omega} + \tpl{\hat{i}}{\omega}), && \tpl{\hat{i}}{\omega} \in \inti{1}{b}^{\omega}\}.
%\end{alignat*}
%%\begin{alignat*}{3}
%%\tilde{B}^{\tpl{I}{t}\tpl{J}{v}}&=\{ 
%%B_{\tpl{i}{t}\tpl{j}{v}} \ | \ 
%%\ \forall \ \tpl{i}{t}=(b\cdot \tpl{I}{t} + \tpl{\hat{i}}{t}),
%%\tpl{\hat{i}}{t} \in \inti{1}{b}^t && \mathrm{\ and \ } 
%%&&\tpl{j}{v} = (b\cdot \tpl{J}{v} + \tpl{\hat{j}}{v}),
%%\tpl{\hat{j}}{v}\in \inti{1}{b}^v \}, \\
%%\tilde{C}^{\tpl{I}{s}\tpl{J}{t}}&=\{ 
%%C_{\tpl{i}{s}\tpl{j}{t}} \ | \
%%\ \forall \ \tpl{i}{s}=(b\cdot \tpl{I}{s} + \tpl{\hat{i}}{s}),
%%\tpl{\hat{i}}{s} \in \inti{1}{b}^s && \mathrm{\ and \ } 
%%&&\tpl{j}{t} = (b\cdot \tpl{J}{t} + \tpl{\hat{j}}{t}),
%%\tpl{\hat{j}}{t}\in \inti{1}{b}^t \}, \\
%%\noalign{\hspace*{-.22in}$\tilde{Z}^{\tpl{I}{s}\tpl{J}{t}\tpl{L}{v}}=\{
%%\hat{Z}_{\tpl{i}{s}\tpl{j}{t}\tpl{l}{v}} \ | \ 
%%\ \forall \ \tpl{i}{s}=(b\cdot \tpl{I}{s} + \tpl{\hat{i}}{s}), \tpl{\hat{i}}{s} \in \inti{1}{b}^s,  \ \ 
%%\tpl{j}{t}= (b\cdot \tpl{J}{t} + \tpl{\hat{j}}{t}),
%%\tpl{\hat{j}}{t}\in \inti{1}{b}^t,$} 
%%& &&  \mathrm{and}  && \tpl{l}{v} = (b\cdot \tpl{L}{v} + \tpl{\hat{l}}{v}),
%%\tpl{\hat{l}}{v}\in \inti{1}{b}^v \}.
%%\end{alignat*}
%We can now reference the elements of the tensors $\C A$, $\C B$, and $\C{\hat{Z}}$ by the block to which they belong
%along with the offset inside the block, as  $\forall \tpl{i}{\omega}\in\inti{1}{n}^\omega, \ \exists \tpl{I}{\omega}\in \inti{0}{n/b-1}^\omega,
%\tpl{\hat{i}}{\omega}\in \inti{1}{b}^\omega$, such that $\tpl{i}{\omega} = b\cdot \tpl{I}{\omega}+ \tpl{\hat{i}}{\omega}$, so
%$$\hat{Z}_{\tpl{i}{\omega}} = \hat{Z}_{b\cdot \tpl{I}{\omega} + \tpl{\hat{i}}{\omega}} = 
%  \tilde{Z}^{\tpl{I}{\omega}}_{\tpl{\hat{i}}{\omega}}.$$
%Now, we express the multiplications necessary to compute $\C{\hat{Z}}$ according to the blocks
%of $\C A$ and $\C B$ whose input they require starting with equation~\ref{eq:fschatZ},
%$\forall \tpl{i}{\omega} = b\cdot \tpl{I}{\omega}+ \tpl{\hat{i}}{\omega}$,
%\begin{align*}
%\hat{Z}_\tpl{i}{\omega} &= \bigg(\sum_{\tpl{j}{ s+v } \in \chi( \tpl{i}{\omega})} A_{\tpl{j}{ s+v }}\bigg) \cdot
%      \bigg(\sum_{\tpl{l}{ v+t } \in \chi( \tpl{i}{\omega})} B_{\tpl{l}{ v+t }}\bigg) \\
%&= \tilde{Z}^\tpl{I}{\omega}_\tpl{\hat{i}}{\omega} = \bigg(\sum_{(b\cdot \tpl{J}{ s+v } + \tpl{\hat{j}}{s+v}) \in \chi( b \cdot \tpl{I}{\omega}+\tpl{\hat{i}}{\omega})} 
%      \tilde{A}^{\tpl{J}{s+v}}_{\tpl{\hat{j}}{ s+v }}\bigg) \cdot
%      \bigg(\sum_{(b\cdot \tpl{L}{v+t} + \tpl{\hat{l}}{ v+t }) \in \chi( b\cdot \tpl{I}{\omega}+\tpl{\hat{i}}{\omega})} \
%      \tilde{B}^{\tpl{L}{v+t}}_{\tpl{\hat{l}}{ v+t }}\bigg), \label{eq:Zblk} \numberthis
%\end{align*}
%where in the partitioning $(b\cdot \tpl{J}{ s+v } + \tpl{\hat{j}}{s+v}) \in \chi( b \cdot \tpl{I}{\omega}+\tpl{\hat{i}}{\omega})$, 
%each value in $\tpl{J}{s+v}$ takes on a value of $\tpl{I}{\omega}$ of the same index (position in the tuple) as the position of 
%the value of $\tpl{\hat{i}}{s+v}$ which is taken on by $\tpl{\hat{j}}{s+v}$. The same applies to
%$(b\cdot \tpl{L}{v+t} + \tpl{\hat{l}}{ v+t }) \in \chi( b\cdot \tpl{I}{\omega}+\tpl{\hat{i}}{\omega})$.
%So for a given block (given value of $\tpl{I}{\omega}$), the number of blocks of $\C A$ and $\C B$ which contain elements that are 
%necessary to compute $\tilde{Z}^\tpl{I}{\omega}_\tpl{\hat{i}}{\omega}$ for all $\tpl{\hat{i}}{\omega}$, is equal to the number
%of unique values $\tpl{J}{s+v}$ and $\tpl{L}{s+v}$ can take on. Since the partition function acts independently on these block
%indices ($\tpl{J}{s+v}$ and $\tpl{L}{s+v}$ are subsets of $\tpl{I}{\omega}$) and the inner-block indices 
%($\tpl{\hat{j}}{s+v}$ and $\tpl{\hat{l}}{s+v}$ are subsets of $\tpl{\hat{i}}{\omega}$), the values which $\tpl{J}{s+v}$ can take on
%are given by the set $\chi^{s+v}(\tpl{I}{\omega})$, while the values which $\tpl{L}{v+t}$ can take on are given by the set
%$\chi^{v+t}(\tpl{I}{\omega})$. These sets have sizes ${\omega \choose {s+v}}={\omega\choose t}$ and ${\omega \choose v+t} = {\omega\choose s}$,
%respectively. Therefore, to compute all elements of a block $\hat{Z}^{\tpl{I}{\omega}}$ for any $\tpl{I}{\omega}$, the size of the inputs
%needed (the number of reads from memory needed) is
%$$\bwcost_\mathrm{in} = {\omega \choose t}\cdot b^{s+v}+{\omega \choose s}\cdot b^{v+t},$$
%since the size of each block of $\C A$ (element of $\C{\tilde{A}}$) is $b^{s+v}$ while the size of each block of $\C B$ (element of $\C{\tilde{B}}$)
%is $b^{v+t}$. 
%
%$\C Z$ and subsequently $\C C$ is computed from $\C{\hat{Z}}$ via equation~\ref{eq:fscZ}.
%We transform equation~\ref{eq:fscZ} (with $\C Z$ replaced by $\C Q$ for notational convenience) 
%into a blocked version by expressing it in terms of the elements of $\C{\tilde{Z}}$ and $\C{\tilde{Q}}$, where the block-tensor $\C{\tilde{Q}}$ is defined as
%\begin{align*}
%\forall &\tpl{I}{s+t}\in \inti{0}{n/b-1}^{s+t},\\ 
%&\tilde{Q}^{\tpl{I}{s+t}}=\{ Q_{\tpl{i}{s+t}} \ | \ \ \forall \  \tpl{i}{s+t} = (b\cdot \tpl{I}{s+t} + \tpl{\hat{i}}{s+t}),  \tpl{\hat{i}}{s+t} \in \inti{1}{b}^{s+t}\}.
%\end{align*}
%Equation~\ref{eq:fscZ} becomes $\forall \tpl{i}{s+t}=b\cdot \tpl{I}{s+t} + \tpl{\hat{i}}{s+t}$,
%\begin{align*} 
%Q_{\tpl{i}{ s+t }} &=  \sum_{\tpl{k}{v}} \hat{Z}_{\tpl{i}{s+t}\tpl{k}{v}} \\
%&= \tilde{Q}^\tpl{I}{s+t}_{\tpl{\hat{i}}{ s+t }} =  \sum_{b\cdot \tpl{K}{v} + \tpl{\hat{k}}{v}} \hat{Z}^{\tpl{I}{s+t}\tpl{K}{v}}_{\tpl{\hat{i}}{s+t}\tpl{\hat{k}}{v}}. \label{eq:Qblk} \numberthis
%\end{align*}
%We now show that by exploiting symmetry in $\C{\hat{Z}}$ only a fraction of the blocks (elements of $\C{\tilde{Z}}$) actually need to be computed,
%with each one being accumulated into ${\omega \choose v}$ blocks of $\C Q$ (elements of $\C{\tilde{Q}}$) corresponding to the 
%blocks $\tilde{Q}^{\tpl{I}{s+t}}$ given by the partitions $(\tpl{I}{s+t},\tpl{K}{v})\in \chi(\tpl{J}{\omega})$.  
%The symmetry of $\hat{Z}$ was formally demonstrated in the proof of Theorem~\ref{thm:arith_cost_fast}.
%It follows that the elements of block $\tilde{Z}^\tpl{I}{\omega}$ are the same (but differently ordered) as those of $\tilde{Z}^\tpl{J}{\omega}$ whenever
%$\tpl{I}{\omega}$ and $\tpl{J}{\omega}$ are equivalent after some permutation of the block indices $\tpl{J}{\omega}=\pi(\tpl{I}{\omega})$. 
%This is true since for any element of the first block, $\tilde{Z}^\tpl{I}{\omega}_\tpl{\hat{i}}{\omega}=\hat{Z}_{b\cdot \tpl{I}{\omega} + \tpl{\hat{i}}{\omega}}$,
% there is an equivalent element  $\tilde{Z}^{\tpl{J}{\omega}}_{\pi(\tpl{\hat{i}}{\omega})}= \tilde{Z}^{\pi(\tpl{I}{\omega})}_{\pi(\tpl{\hat{i}}{\omega})}=\hat{Z}_{\pi(b\cdot \tpl{I}{\omega}+\tpl{\hat{i}}{\omega})}$,
%due to the fact that $\C{\hat{Z}}$ is symmetric (symmetry means that for any permutation of indices $\pi'$, $\hat{Z}_{\tpl{i}{\omega}}=\hat{Z}_{\pi'(\tpl{i}{\omega})}$).
%Now, since $\C Q=\C Z$ is symmetric, it similarly follows that the elements of each block $\tilde{Q}^{\tpl{I}{s+t}}$ are the same as of any block
%$\tilde{Q}^{\tpl{J}{s+t}}$ when $\tpl{I}{s+t}$ and $\tpl{J}{s+t}$ are equivalent after permutation. Therefore, it suffices to compute only blocks
%$\tilde{Q}^{\tpl{I}{s+t}}$ where $\tpl{I}{s+t}$ is in normal order ($I_1\leq I_2 \leq \ldots I_{s+t}$). Further, these blocks of $\C Q$ can be computed 
%from only the blocks of $\tilde{Z}^\tpl{J}{\omega}$ for which $\tpl{J}{\omega}$ is in normal order. In particular, whenever our schedule computes
%each normal-ordered block, $\tilde{Z}^\tpl{J}{\omega}$, it accumulates the block to all normal-ordered blocks of $\C Q$ to which certain permutations of the
%indices $\tpl{J}{\omega}$ contributes. These permutations correspond to partitions of the index set $\tpl{J}{\omega}$ into $\tpl{I}{s+t}$ and $\tpl{K}{v}$, which
%are given by the set $\chi^{s+t}_v(\tpl{J}{\omega})$, the size of which is $\omega \choose v$. 
%So, for each block of $\C{\hat{Z}}$ the schedule computes, it accumulates to memory (which we allow to be done with a unit memory transfer cost) 
%$$\bwcost_\mathrm{out} = {\omega \choose v}\cdot b^{s+t},$$
%elements of $\C Q$, since each block of $\C Q$ is of size $b^{s+t}$. 
%
%\begin{algorithm} 
%%\caption{Krylov subspace bandwidth-efficient parallelization} 
%\begin{algorithmic}[1]
%%\caption {$	ext{PA3}(V_\mathrm{Kr},n,m,d,H,p)$} 
%%\State \Comment assume $p^{1/d}$ is an integer and $m\leq \frac{1}{2}(H\cdot p)^{1/d}$
%\caption {$\C{\tilde{Q}} \gets 	\mathrm{symmetric-schedule}(\C{\tilde{A}}, \C{\tilde{B}}, s,t,v)$}
%\label{alg:Zalg}
%\For {{\bf all} $\tpl{I}{s+t}\in\inti{0}{n/b-1}^\omega$, such that $I_1\leq I_2\leq\ldots I_{s+t}$ }
%  \State Initialize block $\tilde{Q}^\tpl{I}{s+t}$ to zero
%\EndFor
%\For {{\bf all} $\tpl{J}{\omega}\in\inti{0}{n/b-1}^\omega$, such that $J_1\leq J_2\leq\ldots J_{\omega}$ }
%  \State Load into cache all blocks $\tilde{A}^\tpl{I}{s+v}$ for all 
%      $\tpl{I}{s+v} \in \chi(\tpl{J}{\omega})$
%  \State Load into cache all blocks $\tilde{B}^\tpl{I}{v+t}$ for all 
%      $\tpl{I}{v+t} \in \chi(\tpl{J}{\omega})$
%  \State Compute all elements in block $\tilde{Z}^{\tpl{J}{\omega}}$ via equation~\ref{eq:Zblk}
%  \For {{\bf all} $(\tpl{I}{s+t},\tpl{K}{v})\in \chi(\tpl{J}{\omega})$ }
%    \State Reorder the elements of $\tilde{Z}^{\tpl{J}{\omega}}$ to obtain
%        the block $\tilde{Z}^{\tpl{I}{s+t}\tpl{K}{v}}$ 
%    \State Let $r$ be the number of unique possible orderings of the set of values in $\tpl{K}{v}$
%    \For {{\bf all} $\tpl{\hat{i}}{s+t} \in \inti{1}{b}^{s+t}$ }
%       \State Accumulate $\tilde{Q}^\tpl{I}{s+t}_\tpl{\hat{i}}{s+t} := \tilde{Q}^\tpl{I}{s+t}_{\tpl{\hat{i}}{s+t}} + 
%      r\cdot \sum_{\tpl{\hat{k}}{v}} \tilde{Z}_{\tpl{\hat{i}}{s+t}\tpl{\hat{k}}{v}}^{\tpl{I}{s+t}\tpl{K}{v}}$
%    \EndFor
%  \EndFor
%\EndFor
%\end{algorithmic}
%\end{algorithm} 
%
%We formulate the above description into Algorithm~\ref{alg:Zalg}.
%We argue that at termination the normal-ordered blocks of $\C Q$ (elements of 
%$\C{\tilde{Q}}$) which Algorithm~\ref{alg:Zalg} computes are equivalent to equation~\ref{eq:Qblk}. 
%Each element, 
%$\tilde{Q}^\tpl{I}{s+t}_{\tpl{\hat{i}}{ s+t }}$ is a sum of $n^v$ elements of
%$\C{\hat{Z}}$, which belong to elements of $(n/b)^v$ blocks, 
%$\tilde{Z}^{\tpl{I}{s+t}\tpl{K}{v}}$, for the $(n/b)^v$ values that $\tpl{K}{v}$
%can take on. We can observe that the contributions to
%$\tilde{Q}^\tpl{I}{s+t}_{\tpl{\hat{i}}{ s+t }}$ of
%$\tilde{Z}^{\tpl{I}{s+t}\tpl{K}{v}}$ and 
%$\tilde{Z}^{\tpl{I}{s+t}\tpl{K'}{v}}$ for any permutationally equivalent
%$\tpl{K'}{v}=\pi(\tpl{K}{v})$ are the same due to the symmetry in $\C{\hat{Z}}$, since
%\begin{align*}
%\sum_{\tpl{\hat{k}}{v}} \tilde{Z}^{\tpl{I}{s+t}\tpl{K'}{v}}_{\tpl{\hat{i}}{s+t}{\tpl{\hat{k}}{v}}} 
%  &= \sum_{\tpl{\hat{k}}{v}} \hat{Z}_{b \cdot \tpl{I}{s+t}\tpl{K'}{v} + \tpl{\hat{i}}{s+t}{\tpl{\hat{k}}{v}}} \\
%  &= \sum_{\tpl{\hat{k}}{v}} \hat{Z}_{(b \cdot \tpl{I}{s+t} + \tpl{\hat{i}}{s+t})(\tpl{K'}{v} + \tpl{\hat{k}}{v})} \\
%  &= \sum_{\pi(\tpl{\hat{k}}{v})} \hat{Z}_{(b \cdot \tpl{I}{s+t} + \tpl{\hat{i}}{s+t})\pi(\tpl{K'}{v} + \tpl{\hat{k}}{v})} \\
%  &= \sum_{\tpl{\hat{l}}{v}} \hat{Z}_{(b \cdot \tpl{I}{s+t} + \tpl{\hat{i}}{s+t})(\tpl{K}{v} + \tpl{\hat{l}}{v})} \\
%  &= \sum_{\tpl{\hat{l}}{v}} \tilde{Z}^{\tpl{I}{s+t}\tpl{K}{v}}_{\tpl{\hat{i}}{s+t}{\tpl{\hat{l}}{v}}}
%\end{align*}
%This equivalence justifies the multiplication by a factor of $r$ in Algorithm~\ref{alg:Zalg} which is the number of unique possible orderings of $\tpl{K}{v}$, since
%by the argument above the contributions of all these blocks for each element of $\C Q$ is the same.
%This factor is different depending on how many values in the index set $\tpl{K}{v}$ are the same (diagonals need
%to be multiplied by different factors, as is also done in the standard algorithm, $\Psi_\odot^{(s,t,v)}(\C A, \C B)$, when $v>1$).
%When $\tpl{K}{v}$ contains $l\leq v$ different values with multiplicities $m_1,m_2,\ldots m_l$, $\sum_{i=1}^l m_i=v$,
%$r$ is a multinomial, which means that $r=v!/\prod_{i=1}^l m_i!$.
%
%We can then argue that all $(n/b)^v$ blocks which contribute to each element of $\C Q$ in equation~\ref{eq:Qblk}
%are accounted for, since for each index to $\C{\tilde{Z}}$ in equation ~\ref{eq:Qblk}, $\tpl{I}{s+t}\tpl{K}{v}$,  we know that
%\begin{itemize}
%\item $\tpl{I}{s+t}$ will be in normal-order since we only compute blocks of $\C Q$ whose indices are in normal order,
%\item there exists a block $\tilde{Z}^{\tpl{I}{s+t}\tpl{K'}{v}}$ where $\tpl{K'}{v}=\pi(\tpl{K}{v})$ for some permutation $\pi$ such that $\tpl{K'}{v}$ is in normal order and
%      whose contribution is the same as that of $\tilde{Z}^{\tpl{I}{s+t}\tpl{K}{v}}$ due to the symmetry argument given above, and there are
%      $r$ such blocks which share the same normal order after permutation (distinct possible orderings of $\tpl{K}{v}$),
%\item there exists a block $\tilde{Z}^\tpl{J}{\omega}$ where $\tpl{J}{\omega}$ is in normal order and permutationally equivalent to 
%      $\tpl{I}{s+t}\tpl{K'}{v}$ ($\exists \pi$, such that $\pi(\tpl{I}{s+t}\tpl{K'}{v})=\tpl{J}{\omega}$),
%\item Algorithm~\ref{alg:Zalg} computes block $\tilde{Z}^\tpl{J}{\omega}$ since it computes all blocks of $\C{\hat{Z}}$ with a normal-ordered index,
%\item Algorithm~\ref{alg:Zalg} adds the correct elements of the block $\tilde{Z}^\tpl{J}{\omega}$ to all elements in $\tilde{Q}^\tpl{I}{s+t}$ 
%      since $(\tpl{I}{s+t},\tpl{K'}{v})\in \chi(\tpl{J}{\omega})$ with the desired prefactor of $r$ accounting for all distinct possible orderings of $\tpl{K'}{v}$.
%\end{itemize}
%%\hat{Z}_\tpl{i}{\tpl{i}{s}\tpl{j}{t}\tpl{l}{v}} = \bigg(\sum_{\tpl{j}{ s+v } \in \chi( \tpl{i}{\omega})} A_{\tpl{j}{ s+v }}\bigg) \cdot
%%      \bigg(\sum_{\tpl{l}{ v+t } \in \chi( \tpl{i}{\omega})} B_{\tpl{l}{ v+t }}\bigg). 
%%\tilde{Z}^{\tpl{I}{\omega}}_{\tpl{i}\omega}&=
%%  \lt(\sum_{(\tpl{J}{s},\tpl{H}{v})\in\chi(\tpl{I}{\omega})} 
%%      \sum_{(\tpl{j}{s},\tpl{h}{v})\in\chi(\tpl{i}{\omega})} 
%%      \tilde{A}^{\tpl{J}{s} \tpl{H}{v}}_{\tpl{j}{s} \tpl{h}{v}}\rt)
%%  \cdot \lt(\sum_{(\tpl{L}{t},\tpl{H}{v})\in\chi(\tpl{I}{\omega})} 
%%  \sum_{(\tpl{l}{t},\tpl{h}{v})\in\chi(\tpl{i}{\omega})} 
%%    \tilde{B}^{\tpl{L}{t} \tpl{H}{v}}_{\tpl{l}{t} \tpl{h}{v}}\rt) \\
%%\tilde{C}^{\tpl{J}{s+t}}_{\tpl{j}{s+t}}&=
%%\sum_{\tpl{J}{s+t}\in\chi(\tpl{I}{\omega})} 
%%\sum_{\tpl{j}{s+t}\in\chi(\tpl{i}{\omega})} 
%%\tilde{Z}^{\tpl{I}{\omega}}_{\tpl{i}{\omega}} + \ldots 
%%\end{align*}
%
%We can quantify the communication cost of Algorithm~\ref{alg:Zalg} by multiplying the number of blocks of $\C{\hat{Z}}$
%it computes by the size of the inputs $\bwcost_\mathrm{in}$ needed to compute the block and adding this to the size of
%the outputs $\bwcost_\mathrm{out}$ to which the result of the block is accumulated.  Only the blocks of $\C{\hat{Z}}$ which
%have normal-ordered indices are computed, and the total number of such blocks is $\chchoose{n/b}{\omega}$.
%Assuming accumulation to memory and reads
%from memory have unit cost and that the inputs and outputs all fit into cache, we then obtain the following expression for 
%the communication cost of Algorithm~\ref{alg:Zalg},
%\begin{align*}
%\bwcost_Z(n,s,t,v,b)&= \chchoose{n/b}{\omega}(\bwcost_\mathrm{in}+\bwcost_\mathrm{out}) \\ 
%&=\frac{n^\omega}{\omega!\cdot b^\omega}\Bigg[
%{\omega \choose t}\cdot b^{s+v}+{\omega \choose s}\cdot b^{v+t}+{\omega \choose v}\cdot b^{s+t}\Bigg] + O(n^{\omega-1})
%\end{align*}
%The amount of cache used by the algorithm throughout the computation of each block of $\C{\hat{Z}}$ is
%$$\bwcost_\mathrm{in}+\bwcost_\mathrm{out}={\omega\choose t}\cdot b^{s+v}+{\omega \choose s}\cdot b^{v+t}+{\omega \choose v}\cdot b^{s+t},$$ 
%which
%we need to be less than the size of the cache $\cachesize$. Therefore, we pick $b$ to be 
%\begin{align*}
%b&=\Bigg(\cachesize/\bigg[{\omega \choose s}+{\omega \choose t} + {\omega \choose v}\bigg]\Bigg)^{1/\max(s+v,v+t,s+t)} 
%%&=\Bigg(\cachesize/\bigg[{\omega \choose s}+{\omega \choose t} + {\omega \choose v}\bigg]\Bigg)^{1/(\omega-\min(s,v,t))}
%\end{align*}
%%=(\cachesize/3\min()^{1/(\omega-\min(s,v,t))}$.
%Substituting this $b$ into $\bwcost_Z(n,s,t,v,b)$, we obtain the following upper bound on the communication cost of Algorithm~\ref{alg:Zalg}
%\begin{align*}
%\bwcost_Z(n,s,t,v,\cachesize)\leq &\frac{n^\omega\cdot \big[{\omega \choose s}+{\omega \choose t} + {\omega \choose v}\big]^{1/\max(s+v,v+t,s+t)}}{\omega!\cdot \cachesize^{\omega/(\max(s+v,v+t,s+t))}}\cdot \cachesize + O(n^{\omega-1}) \\
%=&\frac{n^\omega \cdot \big[{\omega \choose s}+{\omega \choose t} + {\omega \choose v}\big]^{1/\max(s+v,v+t,s+t)}}{\omega!\cdot \cachesize^{-1+\omega/\max(s+v,v+t,s+t)}} + O(n^{\omega-1})
%\end{align*}
%We now consider the communication costs associated with computing the other intermediates, $\C{A^{(r)}}$, $\C{B^{(r)}}$, $\C V$, $\C{U^{(r)}}$, and $\C W$.
%As we noted in the proof of Theorem~\ref{thm:arith_cost_fast} the number of operations required to compute these is $O(n^{\omega-1})$ whenever $s,v,t>0$,
%so the communication cost in this case is also bound by $O(n^{\omega-1})$. When $v=0$, computing $\C W$ is no longer a low-order cost, but we can
%bound it by $O(n^{s+t})$ (since this is a bound on the number of operations needed to compute $\C W$), 
%which also bounds the cost of writing the results into the output $\C C$. In the cases when either $s=0$ or $t=0$, the computation of $\C{B^{(1)}}$ and 
%$\C{A^{(1)}}$, respectively, become leading order terms. We can, however, also bound these costs by the size of the inputs $O(n^{s+v}+n^{v+t})$.
%Combining these bounds with the bound for Algorithm~\ref{alg:Zalg}, which computes $\C Z= \C Q$, yields the following upper bound on the 
%communication cost of the fast tensor contraction algorithm:
%\begin{align*}
%\bwcost^\Phi(n,s,t,v,\cachesize)&= 
%\frac{n^\omega \cdot \big[{\omega \choose s}+{\omega \choose t} + {\omega \choose v}\big]^{1/\max(s+v,v+t,s+t)}}{\omega!\cdot \cachesize^{-1+\omega/\max(s+v,v+t,s+t)}}  + O(n^{s+t} + n^{s+v} + n^{v+t} + n^{\omega-1}).
%\end{align*}
%%
%%
%%
%%Since $b\ll n$, the number of blocks $\C{\tilde{Z}}^{\tpl{I}{\omega}}$ which contain
%%some entry of $\C{\hat{Z}}$ that is in normal order ($\hat{Z}_\tpl{j}{\omega}$ with $j_1\leq j_2\leq \ldots j_\omega$),
%%is the number of unique entries of $\C{\hat{Z}}$ divided by the volume of each
%%$\C{\tilde{Z}}$ block, $\frac{n^\omega}{\omega!b^\omega}+O(n^{\omega-1})$. In other words,
%%this is the number of blocks necessary to cover all unique entries of $\C{\hat{Z}}$. Each block in
%%$\C{\tilde{Z}}$ depends on $\omega\choose t$ blocks in $\C{\tilde{A}}$, $\omega \choose s$ blocks in
%%$\C{\tilde{B}}$ and contributes to $\omega \choose v$ blocks of $\C{\tilde{C}}$. The total amount of entries in
%%each block of $\C{\tilde{Z}}$ is dependent on and a dependency of is given by
%%$$\tilde{M}=
%%{\omega \choose t}\cdot b^{s+v} +
%%{\omega \choose s}\cdot b^{v+t} +
%%{\omega \choose v}\cdot b^{s+t}$$
%%If all of these blocks fit in cache for each block of $\C{\tilde{Z}}$, namely if $M\leq \tilde{M}$ 
%%the communication cost is 
%%$$\frac{n^\omega}{\omega!b^\omega}\cdot 
%%\lt({\omega \choose t}\cdot b^{s+v} +
%%{\omega \choose s}\cdot b^{v+t} +
%%{\omega \choose v}\cdot b^{s+t}\rt) + O(n^{\omega-1}).$$
%%Now, choosing $b=(M/3)^{1/\max(s+v,v+t,s+t)}$
%%we obtain the following bandwidth
%%cost for computing $\C Z$ via this schedule,
%%\begin{align*}
%%\frac{n^\omega}{\omega!(M/3)^{\omega/\max(s+v,v+t,s+t)}}\cdot 
%%\Bigg(&{\omega \choose t}\cdot (M/3)^{(s+v)/\max(s+v,v+t,s+t)} +
%%{\omega \choose s}\cdot (M/3)^{(v+t)/\max(s+v,v+t,s+t)} + \\
%%&{\omega \choose v}\cdot (M/3)^{(s+t)/\max(s+v,v+t,s+t)}\Bigg) + O(n^{\omega-1}) \\
%%&\leq \frac{n^\omega}{\omega!(M/3)^{\omega/\max(s+v,v+t,s+t)-1}}\cdot 
%%\lt({\omega \choose t} +
%%{\omega \choose s} +
%%{\omega \choose v}\rt) + O(n^{\omega-1}) 
%%\end{align*}
%%The number of operations required for computing $\C W$ and $\C V$ is either
%%on the order of $n^{\omega-1}$ or in the case when one of $s,v,t$ is zero the number
%%of additions is leading order, but no more than the size of one of the inputs (FIXME account for W)
%%or outputs, so all together no more than $\frac{n^{s+v}}{(s+v)!}+ \frac{n^{v+t}}{(v+t)!} + \frac{n^{s+t}}{(s+t)!}$. We can therefore upper-bound the 
%%communication cost of the algorithm as
%%\begin{align*}
%%W^\Phi(n,s,t,v,M)&= \frac{n^\omega/\omega!}{(M/3)^{\omega / \max(s+v,v+t,s+t)-1}}\cdot
%%                        \lt[{\omega\choose t} 
%%                            +{\omega\choose s} 
%%                            +{\omega\choose v} \rt] + \frac{2n^{s+v}}{(s+v)!}+ \frac{2n^{v+t}}{(v+t)!} + \frac{2n^{s+t}}{(s+t)!} +
%%                            O(n^{\omega-1}).
%%\end{align*}
%%
%{\bf Lower bound:}


%Now we prove 
A previous proof of these communication lower bound on algorithm $\syfsalg ABstv$ appeared in \cite{ES_dissertation_2014}.
It employed the lower bound technique from Christ et al.~\cite{christ2013communication}, which relies on the 
H\"older inequality~\cite{Holder1889} and its generalization~\cite{bennett2008brascamp}.
More specifically, it employed Theorem 6.6 
from Section 6.3 of Christ et al.~\cite{christ2013communication}, which applies to programs which are 
loop nests where in the innermost loop arrays are accessed based on subsets of the loop indices. 
In this version, we simplify the proof by employing the generalized Loomis-Whitney inequality~\cite{Tiskin98thedesign} (Lemma~\ref{thm:tlw}). 
%$\syfsalg ABstv$ %Algorithm~\ref{alg:Znorm} 
%\fixme{Edgar}{This used to be a for loop alg.} is exactly this type of program, with $\omega$
%nested loops and with ${\omega \choose t}$ accesses to the $\C{A}$ array, ${\omega \choose s}$
%accesses to the $\C{B}$ array, and ${\omega \choose v}$ accesses to the $\C{Z}$ array in the innermost loop.
%Each of these ${\omega \choose t} + {\omega \choose s} + {\omega \choose v}$ accesses
%is a projection or homomorphism in the language of~\cite{christ2013communication}, which
%is a mapping from the index set $\tpl{i}{\omega}$ to a subset thereof. We enumerate these
%homomorphisms for accesses to $\C A$ by enumerating the set $\chi^{s+v}(\tpl{i}{\omega})$, with
%$\phi^A_j(\tpl{i}{\omega})$ being the $j$th member of the set for $j\in\inti{1}{\omega \choose t}$.
%We similarly enumerate the access to $\C B$ by enumerating the set $\chi^{v+t}(\tpl{i}{\omega})$, with
%$\phi^B_j(\tpl{i}{\omega})$ being the $j$th member of the set for $j\in\inti{1}{\omega \choose s}$.
%Lastly, we enumerate the accesses (accumulates) to $\C Z$ by enumerating the set 
%$\chi^{s+t}(\tpl{i}{\omega})$, with
%$\phi^B_j(\tpl{i}{\omega})$ being the $j$th member of the set for $j\in\inti{1}{\omega \choose v}$.
%Now, we ignore two of the three of these sets of projections (ignoring some dependencies still allows
%us to obtain a valid lower bound in this case), namely we pick $r=\min(s,v,t)$, then if $r=t$ we take the 
%projections from $\C A$, otherwise if $r=s$ we take the projections from $\C B$, 
%and if $r<s,t$, so $r=v$, we take the
%projections from $\C Z$. We end up with projections $\phi_j(\tpl{i}{\omega})$, which enumerate
%the set $\chi^{\omega-r}(\tpl{i}{\omega})$ for $j\in\inti{1}{\omega \choose r}$.
%
%We would like to use the implication of Theorem 3.2 of~\cite{christ2013communication}, which
%states that if the projections $\phi_j$ for $j\in \inti{1}{\omega \choose r}$ satisfy a
%certain constraint for parameters $s_j\in [0,1]$, then given any set of index tuples 
%(loop iterations) $E=\{\tpl{i}{\omega} \in \inti{1}{n}^{\omega}\}$,
%\begin{align*}
%|E|\leq \prod_{j=1}^{\omega \choose r}|\phi_j(E)|^{s_j} \numberthis \label{eq:hblineq}
%\end{align*}
%So, the exponents $s_j$ bound the amount of iterations which may be computed with a given
%set of inputs or outputs based on the projection of the iteration set onto the inputs or outputs.
%The constraint which binds the choice of $s_j$ is significantly simplified from 
%Theorem 3.2 of~\cite{christ2013communication} by Theorem 6.6 of~\cite{christ2013communication}, which 
%applies for our program. In our case, the constraint is (taking the form from the proof of the theorem),
%\begin{align*}
%\forall k\in \inti{1}{\omega}, \ \  \sum_{j=1}^{\omega \choose r}s_j \Delta_{jk} \geq 1, \numberthis \label{eq:hblconst}
%\end{align*}
%where $\C{\Delta}$ is an ${\omega\choose r}$-by-$\omega$ matrix, with
%$\Delta_{jk}=1$ if $i_k\in \phi_j(\tpl{i}{\omega})$ and $\Delta_{jk}=0$ otherwise.
%In our case, $\C \Delta$ has $\omega-r$ ones per row, since each $\phi_j$ takes a distinct
%subset of $\omega-r$ indices. Further, since each index appears in the same number of subsets
%(elements of the set $\chi^{\omega-r}(\tpl{i}{\omega})$), the number of ones per column in $\C \Delta$ 
%is balanced and therefore equal to the number of ones per row multiplied by the number of rows
%and divided by the number of columns, 
%$$\sum_{j=1}^{\omega \choose r} \Delta_{jk} = (\omega-r) {\omega\choose r}/\omega = {\omega -1 \choose r-1}.$$
%So, we can satisfy the constraint in equation~\ref{eq:hblconst} by selecting 
%$s_j=1/{\omega -1 \choose r-1}$ for all $j\in \inti{1}{\omega \choose r}$.

Any sequential schedule $\mathcal S$ must compute $\chchoose{n}{\omega}=|\enti 1n\omega|$ multiplications involved in forming $\BH Z$ \eqref{eq:fscmul} in $\syfsalg ABstv$. %iterations of Algorithm~\ref{alg:Znorm},
We subdivide the schedule into $f+1$ intervals, such that during each interval $\mathcal S_i$ for $i\in\inti 1f$ a set of $\BH Z$ elements is computed with indices in $E_i\subseteq \enti 1n\omega$ such that
$|E_i|=(2\cachesize)^{\omega/\kappa},$
where $\kappa \defeq \max(s+v,v+t,s+t)$.
%ordering into intervals, each defined by a set of $\omega$-tuples corresponding to the computed multiplications:
%\[\{E_i\subset |\enti 1n\omega| : \in\inti{1}{f}, f=\lceil\chchoose{n}{\omega}/(2\cachesize)^{\omega/(\omega-r)}\rceil.\]
%The first $f-1$ sets are of size $(2\cachesize)^{\omega/(\omega-r)}$ while the last remainder 
The last remainder interval $\mathcal S_{f+1}$ computes the rest of the elements of $\BH Z$ with indices $E_{f+1}$,
%subset of size 
\begin{align*}
|E_{f+1}|&=\chchoose{n}{\omega}-(2\cachesize)^{\omega/\kappa} \left\lfloor \chchoose{n}{\omega}/(2\cachesize)^{\omega/\kappa}\right\rfloor\leq (2\cachesize)^{\omega/\kappa}.
\end{align*}
%which may be zero.
%We assume $(2M)^{\omega/(\omega-r)}$ does not divide evenly into the number of total iterations, since the other
%case is strictly simpler. 
%Now, for each $E_i$ we have the bound from~\eqref{eq:hblineq},
%\begin{align*}
%|E_i|&\leq \prod_{j=1}^{\omega \choose r}|\phi_j(E_i)|^{s_j} \leq \prod_{j=1}^{\omega \choose r}|\phi_j(E_i)|^{1/{\omega-1 \choose r-1}}.
%\end{align*}
We obtain a lower bound on the number of reads from cache and writes to cache done by each $S_i$.%  by considering two cases, {\bf case (I)}: $s>v$ or $t>v$ and {\bf case (II)}: $v\geq s,t$.

\fixme{Edgar}{Use Lemmas for following.}

{\bf Reads:} %$v\geq s,t$. 
%In the first case, the size of the inputs $\C A$ and $\C B$ is larger than the size outputs ($\C C$ and also $\C Z$ in \eqref{eq:fscZ}).
%Assume without loss of generality that $s \geq t$, which implies $\C A$ is at least as large as $\C B$.
For each $\tpl{i}{\omega}\in E_i$, an element $\hat{Z}_\tpl{i}{\omega}$ is computed via $\hat{A}_\tpl{i}{\omega}$, which consists of $A_{\tpl j{s+v}}$ for all $\tpl j{s+v}\in L_i^\mathrm{in}$, where
\[L_i^\mathrm{in}=\{\tpl{j}{ s+v } : \tpl{j}{ s+v } \in \prj{s+v}( \tpl{i}{\omega}), \tpl i\omega \in E_i\}.\]
By Lemma~\ref{thm:tlw} with $r=s+v$ and $m=\omega$, the size of this set of dependencies is at least $|L_i^\mathrm{in}|\geq |E_i|^{(s+v)/\omega}$.
The elements of $E_i$ can also be computed from partial sums, but by assumption, each would require a unique partial sum, so a set of dependencies with partial sums 
replacing corresponding elements of $\B A$ would be of size only greater than $|E_i|^{(s+v)/\omega}$. 
The argument above can also be made for the $\hat{B}_\tpl{i}{\omega}$ operand needed by $\hat{Z}_\tpl{i}{\omega}$, so we assert %that whenever $v\geq s,t$
there is a set of dependencies with indices $L_i^\mathrm{in}$, such that $|L_i^\mathrm{in}|\geq |E_i|^{\max(s+v,v+t)/\omega}$.
Now, at the start of the computation of interval $\mathcal S_i$, up to $\cs$ elements with indices $R_i\subseteq L_i$ may be in cache, the rest of the elements with indices $\breve{L}^\mathrm{in}_i=L^\mathrm{in}_i\setminus R_i$,
must be read from memory during interval $\mathcal S_i$. The number of elements read, $\bwcost_i^\mathrm{in}=|\breve{L}^\mathrm{in}_i|$ is
\[\bwcost^\mathrm{in}_i \geq |L^\mathrm{in}_i|-\cs \geq |E_i|^{\max(s+v,v+t)/\omega} - \cs.\]

{\bf Writes:} 
%In the second case, the size of the outputs $\C C$ and also $\C Z$ \eqref{eq:fscZ} is larger than the size of the inputs $\C A$ and $\C B$,
%so we consider the communication necessary for computing the elements of $\C Z$ from $\BH Z$ via \eqref{eq:fscZ}.
%We consider any order of summations in \eqref{eq:fscZ}.
The scalar multiplications corresponding to the set of tuples $E_i$ compute a set of elements of $\BH Z$.
Each of these elements $\hat{Z}_\tpl{i}{\omega}$ contributes to the summation computing $Z_\tpl{h}{s+t}$, for all $\tpl{h}{s+t} \in\prj{s+t}(\tpl i\omega)$ in \eqref{eq:fscZ} (as shown by the reformulation in \eqref{eq:fscZacc}).
Since we assume no recomputation, the schedule interval $\mathcal S_i$ may only discard the element $\hat{Z}_\tpl{i}{\omega}$ if after the interval $E_i$, it has been accumulated into a partial
sum for each such $Z_\tpl h{s+t}$ (we have also assumed these partial sums cannot be reused for different elements of $\B Z$).
We now obtain a bound on the set of outputs of interval $\mathcal S_i$, $L_i^\mathrm{out}$.
We assume without loss of generality that all elements of $\C Z$ computed in $\mathcal S_i$ are accumulated to partial sums $\bar{Z}_\tpl h{s+t}$ for all $\tpl h{s+t} \in L_i^\mathrm{out}$ where
\[L_i^\mathrm{out}=\{\tpl h{ s+t } : \tpl h{ s+t } \in \prj{s+t}( \tpl{i}{\omega}), \tpl i\omega \in E_i\},\]
otherwise the number of outputs is only greater, as each $Z_\tpl i\omega$ that is not accumulated in this way, would need to be an output.
Therefore, by Lemma~\ref{thm:tlw} with $r=s+t$ and $m=\omega$, the size of this set of outputs is at least $|L_i^\mathrm{out}|\geq |E_i|^{(s+t)/\omega}$.
Now, at the end of the interval $\mathcal S_i$, up to $\cs$ of these partial sums with indices $R_i\subseteq L_i$ may remain cache, the rest of the partial sums with indices $\hat{L}^\mathrm{out}_i=L^\mathrm{out}_i\setminus R_i$
must be written to memory during $\mathcal S_i$. The number of such elements written, $\bwcost_i^\mathrm{out}=|\hat{L}^\mathrm{out}_i|$ is
\[\bwcost^\mathrm{out}_i \geq |L^\mathrm{out}_i|-\cs \geq |E_i|^{\max(s+t)/\omega} - \cs.\]

Combining the reads and writes, we conclude that for any interval $\mathcal S_i$, $\bwcost_i=\max(\bwcost_i^\mathrm{in},\bwcost_i^\mathrm{out})$ elements need to be communicated between memory and cache, 
%\[\bwcost_i = \max(\bwcost^\mathrm{in}_i,\bwcost^\mathrm{out}_i) \geq |E_i|^{\max(s+v,v+t,s+t)/\omega} - \cs = |E_i|^{\kappa/\omega}-\cs.\]
\[\bwcost_i \geq |E_i|^{\max(s+v,v+t,s+t)/\omega} - \cs = |E_i|^{\kappa/\omega}-\cs.\]
For $i\in \inti{1}{f}$, we can plug in $|E_i|=(2\cachesize)^{\omega/\kappa}$ to obtain 
\[\bwcost_i \geq \cs.\]


% is bound by the cache size $\cachesize$ 
%(partial sums kept in cache at the end of segment) added to the number of writes/accumulates done 
%to memory $\bwcost_i$ during segment $i$ for $i< f$, since we %$\lceil\chchoose{n}{\omega}/(2\cachesize^{\omega/(\omega-r)})\rceil$, since we
%assume no recomputation, meaning all partial sums computed in the last chunk have to be written to memory during the last chunk.
%However, if we are considering projections onto $\C A$ or $\C B$, the size of each $\phi_j(E_i)$ would be
%bound by the cache size $\cachesize$ (operands from the previous segment) added to the number of reads from memory $\bwcost_i$ done during chunk $i$ for
%all $i> 1$ and exclusively $\bwcost_i$ for $i=1$, since we assume the cache begins empty. 
%We note that in these latter cases (operand projections), we can consider the schedule ordering in reverse so that the remainder chunk be the last chunk
%in reverse order (first chunk actually executed), the bounds on $\phi_j(E_i)$ become the same as in the case when
%we are considering projections of the partial sums to $\C Z$. So, without loss of generality, we assume the bounds $\phi_j(E_i)\leq \cachesize+\bwcost_i$
%for all $i<f$ and $\phi_j(E_f)\leq \bwcost_f$. We now seek to obtain a lower bound on communication cost by obtaining a lower bound on
%$\sum_{i=1}^f \bwcost_i$. We ignore the remainder chunk and obtain a bound for each $i\in \inti{1}{f-1}$,
%\begin{align*}
%|E_i|&\leq \prod_{j=1}^{\omega \choose r}|\phi_j(E_i)|^{1/{\omega-1 \choose r-1}}, \\
%(2\cachesize)^{\omega/(\omega-r)}&\leq (\cachesize+\bwcost_i)^{{\omega \choose r}/{\omega-1 \choose r-1}} \\
%                        &= (\cachesize+\bwcost_i)^{\omega/(\omega-r)} \\
%2\cachesize                      &\leq \cachesize+\bwcost_i, \\
%\bwcost_i & \geq \cachesize
%\end{align*}
We can then obtain a lower bound on the communication cost for $\syfsalg ABstv$ by summing over the communication costs of the first $f$ schedule intervals,
%\fixme{Edgar}{This used to use a for loop alg.}, by summing over the $f-1$ iterations of full chunks,
%\begin{align*}
\[\bwcost_\Phi(n,s,t,v,\cachesize)\geq f \cachesize = %\left\lfloor\chchoose{n}{\omega}/(2\cachesize)^{\omega/(\omega-r)}\right\rfloor \cachesize \\
    \left\lfloor\chchoose{n}{\omega}/(2\cachesize)^{\omega/\kappa}\right\rfloor \cachesize.\]
%\end{align*}
\fixme{Edgar}{Clarify.}
We augment this lower bound, by combining it with a lower bound that is based purely on the size of $\C A$ and $\C B$, each of whose entries
must be read into cache at least once and $\C C$, whose entries must be written to memory at least once, obtaining the lower bound stated in the theorem.
%\begin{align*}
%\bwcost_\Phi(n,s,t,v,\cachesize)\geq  \max\Bigg(&\left\lfloor\chchoose{n}{\omega}/(2\cachesize)^{\omega/\kappa}\right\rfloor \cachesize, \\
%                                  &  \frac{n^{s+t}}{(s+t)!}+ \frac{n^{s+v}}{(s+v)!}+ \frac{n^{v+t}}{(v+t)!}\Bigg).
%\end{align*}
\end{proof}


%\begin{theorem}
%The communication cost of computing intermediate tensors 
%$\C Z$, $\C V$, and $\C W$ then forming $\C C$ via 
%equations~\ref{eq:fscZ}--\ref{eq:fscC} given a cache of size $M$ is at most
%\begin{align*}
%\end{align*}
%\end{theorem}
%\begin{proof}
%\end{proof}

We observe that communication cost of the symmetry preserving  algorithm achieves asymptotically
less reuse than the standard algorithm when $s,t,v>0$ and $s,t,v$ are unequal, and so $\omega<(3/2)\kappa$.
In these cases the exponent on $\cachesize$ corresponding to the cache reuse obtained
for each element by the symmetry preserving  algorithm is $\cs^{(\omega/\kappa)-1}<\cs^{1/2}$ (the
standard algorithm gets $\cachesize^{1/2}$ reuse in these case). In the cases when one of 
$s,t,v$ is zero, reading in one of the input tensors or writing the output tensor 
becomes the asymptotically dominant cost for both algorithms. When $s=t=v>0$,
$\syfsalg ABstv$ achieves the same asymptotic reuse factor of $\cachesize^{1/2}$.
% and performs
%less communication by a constant factor due to performing a factor of $\omega!/(s!t!v!)$
%less operations, albeit the benefit in communication does not achieve this full constant
%factor reduction (there is an $\omega!$ in the denominator, but additional, smaller constant
%factors in the numerator) since it requires more communication per computation.

Further, when the algorithm is applied in nested form for partially symmetric contractions~\cite{SD_ETHZ_2015},
%in many of the key applications of the algorithm, where 
each scalar multiplication  done by the symmetry preserving  algorithm can be asymptotically more expensive than each scalar
addition (e.g. a matrix multiplication). In such cases, the reduction in the number of multiplications by $\omega!/(s!t!v!)$
could yield a reduction in communication cost by the same factor, since the underlying scalar 
operation (e.g. matrix multiplication) may achieve a factor of $\cachesize^{1/2}$ reuse itself.
The communication cost analysis done in this section does not correctly capture the cost
in such cases, since it assumes elements of $\C A$, $\C B$, and $\C C$ are all of unit size.



==> tables.tex <==


